Deep Feature-specific Imaging

Modern photon-counting sensors are increasingly dominated by Poisson noise, yet conventional feature-specific imaging (FSI), based on principal component analysis (PCA), is optimized for additive Gaussian noise and variance preservation rather than task-specific objectives, leading to suboptimal performance and a loss of its advantages under Poisson noise. To address this, we introduce DeepFSI, what we believe to be a novel end-to-end optical-electronic framework. DeepFSI "unfreezes" PCA-derived masks, enabling a deep neural network to learn globally optimal measurement masks by computing gradients directly under realistic Poisson and additive noise conditions. Simulations and hardware experiments demonstrate that DeepFSI achieves improved classification accuracy and stronger transfer robustness compared to PCAbased FSI across varying photon budgets, particularly in Poisson-noise-dominant environments. DeepFSI also exhibits enhanced robustness to design choices and performs well under additive Gaussian noise, representing a significant advance for noise-robust computational imaging in photon-limited applications.

==> hardware_pca_onn__Main__authorship <==
\makeatletter
\newcommand{\linebreakand}{%
  \end{@IEEEauthorhalign}
  \hfill\mbox{}\par
  \mbox{}\hfill\begin{@IEEEauthorhalign}
}
\makeatother

\IEEEoverridecommandlockouts

\author{
\IEEEauthorblockN{Yizhou Lu}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: ylu289@wisc.edu}
\and
\IEEEauthorblockN{Trevor Seets}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: seets@wisc.edu}
\and
\IEEEauthorblockN{Ehsan Ahmadi}
\IEEEauthorblockA{Department of Electrical \\and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: eahmadi2@wisc.edu}

% \and
\linebreakand 
\IEEEauthorblockN{Felipe Gutierrez-Barragan}
\IEEEauthorblockA{Department of Computer Sciences\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: fgutierrez3@wisc.edu}
\and
\IEEEauthorblockN{Andreas Velten \thanks{\IEEEauthorrefmark{4} Andreas Velten is corresponding author.}}
\IEEEauthorblockA{Department of Biostatistics and Medical Informatics\\
Department of Electrical and Computer Engineering\\
University of Wisconsin-Madison\\
Madison, Wisconsin 53706\\
Email: velten@wisc.edu}
}

==> hardware_pca_onn__Main__custom_pdfplot_style <==
% plot in latex
\usepackage{pgfplots}
\pgfplotsset{width=10cm,compat=1.9}
% We will externalize the figures
\usepgfplotslibrary{external}
\tikzexternalize
\pgfplotsset{compat=1.18} % Use latest if possible
\usepackage{sansmath} 

\def\axisFont{\fontfamily{cmr}\small}
\def\axisFont{\sffamily\small}



\newenvironment{myaxis}[1][]{
        \begin{axis}[                        
            grid=major,
            legend style={
                at={(0.,0)},anchor=south west, fill opacity=1, 
                % draw=true, 
                font=\axisFont\footnotesize,
                % legend columns=2,     % <- Make it two columns
                % column sep=5pt,
                % row sep=2pt                
                },
            width=.95\linewidth,
            height=.75\linewidth,
            % title={},
            ticklabel style={font=\axisFont\small},
            label style={font=\axisFont\small},
            title style={font=\axisFont},
            #1
        ]
        }{\end{axis}}

==> hardware_pca_onn__Main__custom_sty_submit <==
% re-define the equation environment
\let\oldequation\equation%
\let\endoldequation\endequation%
% \renewenvironment{equation}%
%   {\linenomath\oldequation}{\endoldequation\endlinenomath}%
\expandafter\let\expandafter\oldequationstar\csname equation*\endcsname%
\expandafter\let\expandafter\endoldequationstar\csname endequation*\endcsname%
\renewenvironment{equation*}%
  {\linenomath\oldequationstar}{\endoldequationstar\endlinenomath}%
  

\newcommand{\B}{\boldsymbol}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IZ}{\mathbb{Z}}

\newcommand{\diag}{\text{diag}}

\usepackage{subcaption}

\newcommand{\totphoton}{\mathfrak{N}}
\newcommand{\photon}{\mathfrak{n}}
% \def\totphoton{\left(\rho\tau\right)}

\newcommand{\totexposure}{\tau} %total expo time
\newcommand{\exposure}{\mathfrak{t}} %expo time for each mask
\newcommand{\flux}{\rho} %photons per second



\newcommand{\Xalign}[1]{\begin{aligned}#1\end{aligned}}

\newcommand{\Xequa}[1]{\begin{equation}\Xalign{#1}\end{equation}}




% \def\Xhide#1{\iffalse#1\fi}
\def\Xhide#1{}

\def\noisy#1{\tilde{#1}}
\def\AGN{\mathcal{N}}
\def\Poisson{\mathcal{P}}
\def\Poisson{\mathrm{Poisson}}

% \usepackage{svg}
\usepackage{graphicx} % include PDF figures
\def\Xpolish#1#2{#2}


\def\bnote#1{\textcolor{blue}{#1}}
\def\rnote#1{\textcolor{red} {#1}}
\def\ynote#1{\textcolor{orange}{#1}}
\def\enote#1{\textcolor{violet}{#1}}
\def\YLnote{\rnote}
\def\FGnote#1{\textcolor{brown}{#1}}

\def\ynote#1{\color{orange} #1 \color{black}}
\def\AVnote{\ynote}
\def\TSnote{\bnote}

\def\Bingnote#1{\color{purple} \textit{{#1}} \color{black}}
% \usepackage{pifont}
% \def\checkednote#1{\ding{51} #1}
% \usepackage{soul}
% \usepackage[normalem]{ulem}
% \usepackage{ulem, lipsum}
% \newcommand\xoutpars[1]{\let\helpcmd\xout\parhelp#1\par\relax\relax}
% \newcommand\soutpars[1]{\let\helpcmd\sout\parhelp#1\par\relax\relax}
% \long\def\parhelp#1\par#2\relax{%
%   \helpcmd{#1}\ifx\relax#2\else\par\parhelp#2\relax\fi%
% }

\usepackage[normalem]{ulem}
\def\checkednote#1{\sout{#1}}

%%%%%%network plot
\usepackage{tikz}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary {shapes.misc}
\usepackage{caption}
\usepackage{amsmath,amsfonts}

%%
% \usepackage{slashbox}

%%%% before submit: uncomment the following, OR changing the value of \peerreview in output.tex 
\ifpeerreview
    \linenumbers\linenumbersep 15pt\relax    
    \def\checkednote#1{} % remove comments
    \def\YLnote{}
\else
    % \linenumbers \linenumbersep 15pt\relax  
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\YLnote{}
\def\checkednote#1{}

==> hardware_pca_onn__sections__1_intro__1_intro_2024_01_03 <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi



\YLnote{poisson is not considered before. we developed a simple vision system to address that and compare the noise models impacts}
\YLnote{https://ieeexplore.ieee.org/document/6637874, https://www.nature.com/articles/srep41435.pdf, https://compphotolab.northwestern.edu/wordpress/wp-content/uploads/2015/04/BeatHadamard.pdf}

\IEEEPARstart{T}{}he projection of \checkednote{information} information from a high-dimensional scene space involving color, timing, polarization, and phase onto a lower-dimensional reconstruction space is crucial step in any imaging and vision device. This projection serves the dual purpose of data reduction to fit the limited number of values that can be digitized and processed by the hardware and the extraction of actionable patterns. This process, often termed coding or multiplexing, is a fundamental and essential aspect of both physical and computational considerations in imaging and vision devices. 
In this project, the primary objective is to optimize coding schemes, with a particular emphasis on selecting the appropriate noise model.

\Xhide{Mathematically, coding, it can be described as a linear operator, $\B{M}$ linking a vectorized incoming light field $\B{x}$ to a vector of light measurements $\B{y}$. }
The \textbf{single-pixel-camera} \Xpolish{demonstrated}{shown} in Fig. \ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}. Supposing the image representation of the field of view (FOV) $\B{x} \in \IR^{N \times 1}$ consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ \Xpolish{projections}{measurements, whose photon counts are denoted as $\B{y} \in \IR^{m \times 1}$}, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where \Xhide{$\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, }$\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the field of view onto the sensor pixel\Xhide{, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts }\cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light from $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-rank, \Xpolish{this model accurately characterizes conventional single-pixel imaging scenarios}{the \Xpolish{FOV}{$\B{x}$} can be reconstructed by $\B{M}^{-1}\B{y}$}. However, even when $m < N$, \Xhide{the model remains effective through the integration of regularization techniques, specifically }{we can still recover the \Xpolish{FOV}{$\B{x}$} via} compressed sensing.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct Measurement Strategy: Raster Scan}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {hardware_pca_onn__figures__Background__RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational Imaging (CI) Strategy: Basis Scan}
        \includegraphics[width=1\linewidth]{hardware_pca_onn__figures__Background__BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

In this work we will study the performance of this camera for different choices of $\B{M}$ under different noise models. \Xhide{The single pixel camera is intended specifically as a toy model that exhibits the more general dimensional reduction problem experienced by all imaging devices. Our goal is to design $\B{M}$ such that it allows us to extract desired information from the scene when combined with digital processing. In other words, we seek to design an end to end vision system and consider both the physical and the digital part of the design. }While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.


%A linear operator with a mask can model most optics, including a lens that forms an image, color filters that provide color resolution, and camera pixels that average incoming light over an exposure time. The digitized vector then is processed computationally to extract the desired information about the scene. For a full rank measurement $\B{M}$, a linear operation $\B{M}^{-1}$ can in principle allow reconstruction of the entire incoming measurement. In the simplest case, where the desired information is directly digitized, $\B{M}$ is a diagonal matrix. However far more elaborate capture and post-processing are being employed and are the basis of diverse fields such as structured illumination imaging, computational imaging (CI) \cite{cossairt2012does} and compressed sensing. The primary benefits of complex codes are the improved signal to noise ratio do to the fact that the corresponding masks transmit more light, as well as the possibility of using fewer masks and thereby reducing the overall complexity of the measurement.



% Coding schemes have been extensively studied, but usually based on low noise scenarios or Additive Gaussian noise (AGN) models. AGN is a linear noise model that allows for rigorous mathematical treatment. It is a good model for the readout and background noise introduced by imperfect measurement hardware of past cameras and sensors. However, with the advancement of optical imaging and single photon sensitive sensor technologies, readout noise is decreasing, and Poisson noise is becoming  dominant in measured imaging data\Xhide{ \cite{harwit1979hadamard}}. While the readout noise level of consumer cameras is approaching single electron levels, many state-of-the-art and emerging sensors technologies, such as Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras, directly measure quantized photon counts and as a result only experience Poisson noise \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}. 
Coding schemes, often developed under signal independent Additive Gaussian Noise (AGN), provide a mathematically tractable framework. While AGN is suitable to model certain types of noise introduced by the measurement device, it does not correctly model Poisson noise\YLnote{\Xhide{even after quantization }\cite{yang2015poisson}}\Xhide{ which is signal-dependent and not avoidable via better sensor fabrication techniques. \Xhide{In almost all modern cameras and sensors, however, Poisson noise is predominant, especially in advanced sensors like Single-photon Avalanche Diode (SPAD), Quanta Image Sensors (QiS), and qCMOS cameras \cite{foord1969PMT, prescott1966PMT, lombard1961PMT}.  }This necessitates a reevaluation of coding strategies tailored to this noise type}.

% Poisson noise is a fundamental physical property of light and arises from the discrete nature of light measurements. It is impossible to spread out a photon measurement over all the open pixels in a mask as the linear model introduced in Equation \ref{eqn:NoiselessMeasurement} assumes. The measurements of $\B{y}$ that equation calls for are therefore impossible. Unfortunately, this has the consequence that the coding and thereby compressed sensing approaches designed to be effective under AGN or noiseless conditions are not recommended under Poisson noise and their use is discouraged in the literature \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Poisson noise, a fundamental property of light, arises due to the discrete and random nature of light measurements. \AVnote{\checkednote{ This sentence doesn't seem to make sense Jan 18, 2024 9:41 AM}}\YLnote{\Xpolish{Unlike the assumptions of the linear model in Eq.  \ref{eqn:NoiselessMeasurement},}{Different from AGN, Poisson noise is discrete}} and it is impossible to distribute a photon measurement across all open pixels in a mask. Consequently, linear reconstruction approaches based on the measurements $\B{y}$ called for by the \YLnote{\Xpolish{quation}{Eq.  \ref{eqn:NoiselessMeasurement}}} are \Xpolish{\Xpolish{unattainable}{unsatisfactory}}{unattainable}\Xhide{ by linear reconstruction approaches}. This renders coding and compressed sensing approaches\YLnote{\checkednote{more about  compressed sensing}}, designed for effectiveness under the AGN or noiseless conditions unsuitable. The literature discourages their use in such scenarios \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. \Xhide{The optimal code, denoted as $\B{M}_P$, for measurements limited by real Poisson noise must converge to $\B{M}_G$ applicable to the optimal code under Additive Gaussian Noise (AGN) or under no noise as the number of measured photons tends toward infinity. However, it is crucial to highlight that, as demonstrated below, $\B{M}_P$ does not necessarily exhibit similarity to $\B{M}_G$ for any finite number of photons.}

\AVnote{\checkednote{The optimal code $\B{M}_P$ for a real Poisson noise limited measurement has to approach the $\B{M}_G$ for a noise-less measurement or one under AGN as the number of measured photons goes to infinity. Crucially, however, as we will show below $\B{M}_P$ does not become similar to $\B{M}_G$ for any finite number of photons.}}

% \YLnote{Harwit et al may not say against compressed sensing, but Van den Broek et al mentioned it}
\Xhide{
\Xpolish{In most of the papers, people optimize the algorithms on reconstruction but keep using random coding \cite{goyal2016performance}. Some other work, such as Feature Specific Imaging (FSI) does optimize the sensing matrices based on some learn-able priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, but how to optimize masks under Poisson noise remains an unsolved problem \cite{neifeld2014optimizing}. Meanwhile, some attempts on matrix optimization based on minimal mutual coherence are not based on Poisson noise model itself \cite{mordechay2014matrixRIP} and is proved defective in this paper.}
{
\AVnote{this seems like it belongs into related work}
In many papers, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance}  \YLnote{need more here}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson}. While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methids explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}. Additionally, attempts at matrix optimization focusing on minimal mutual coherence lack a foundation in the Poisson noise model, as highlighted in this study \cite{mordechay2014matrixRIP}.}
}


\Xhide{\Xpolish{Though some signal components must be removed when denoise the Poisson noise, it is possible to selectively keep significant signal components for downstream tasks such as correlation analysis and classification. This kind of coding strategies are called selective sensing (SS) in this paper. When the signal is extremely sparse, SS can have a significant performance gain on the downstream tasks.}
{\Xhide{In this project, we use the popular single pixel camera design to analyze and design effective coding models under Poisson noise. } Therefore, we propose a coding methodology called \textbf{Selective Sensing} (SS) \Xpolish{that relies on finding codes in basis where the signal is sparse and compressible to be used at capture time}{specifically optimized for Poissonian data}. This approach proves particularly effective for extremely sparse and compressible signals such as character recognition, as it enables the retention of key information while reducing the impact of Poisson noise on downstream analyses.}
}%hide old versions
\AVnote{\checkednote{velten: This still comes out of nowhere. So far we have mostly talked about image reconstruction and reconstructing and image x. Now we talk about a vision problem and character recognition.
Maybe Figire 1 should have another component after x that is the output of the vision system or the pattern. That could also be an image. Or we have to say that x is not necessarily and image but could be something else.
Jan 18, 2024 9:50 AM}}
\YLnote{Alternatively, we propose a coding methodology called \textbf{Selective Sensing} (SS) specifically optimized for Poissonian data acquisition. SS focuses on the retention of the key information from some prior knowledge and reducing the impact of Poisson noise for the downstream computer vision tasks, e.g. classification, instead of general reconstruction of $\B{x}$. Its classification performance most closely approaches the theoretical upper limit among all imaging strategies.
}





Our contributions are as listed.
\begin{itemize} 
\item We analyze the performance of coding techniques using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding provides no benefit over a trivial raster scanning approach using a diagonal matrix $\B{M}$ {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits to those seen in compressed sensing and computational imaging can be seen if appropriate adjustments to the measurement matrices are made. 
\item We find\Xhide{, however} that coding can provide significant performance gains \textit{only} when codes used in hardware capture are optimized specifically for downstream image reconstruction or vision tasks, such as classification. 
\item We propose the concept of selective sensing (SS) which includes coding methods selectively extracting the features directly for downstream tasks.
\item We provide a method to create masks optimized for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel cameras.}
\end{itemize}

\Xhide{\Xpolish{While our work is related to compressed sensing and can be applied to regularized image reconstruction where signals are somewhat compressible, we will focus our treatment on two more extreme cases. We will look at cases where data is not compressible and full rank measurements are taken and reconstructed without regularization. On the other extreme we will look at highly compressible data in the problem of image classification where images are projected into a very small feature space. In this highly compressible case, the implications of Poisson noise are the most obvious.}
{
Our work, although rooted in compressed sensing principles applicable to regularized image reconstruction, specifically addresses two extreme scenarios. The first involves non-compressible data with full-rank measurements, reconstructed without regularization. Conversely, we examine highly compressible data in image classification, projecting images into a minimal feature space where the impact of Poisson noise becomes particularly evident.}
\AVnote{\checkednote{Add a figure showing different vision tasks with different compressibilities}}}





==> hardware_pca_onn__sections__1_intro__1_intro_2024_03_02 <==
% The very first letter of the paper is a 2 line initial drop letter
% followed by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi


\IEEEPARstart{O}{}ptical coding, also known as multiplexing, is a \Xpolish{prevalent}{popular} technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput thank point by point measurements\cite{mitra2014can}. The recovery quality of images, however, also depends on the conditioning of the coding matrices \cite{mitra2014can}. Suboptimal coding matrices have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes is intricately linked to the characteristics of noise, a facet that has not been extensively emphasized previously. Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents Poisson noise \cite{yang2015poisson} arising intrinsically due to the discrete and random nature of light measurements. The optimization behaviors of coding manifest notable distinctions under low-light conditions where Gaussian noise dominates and high-light conditions where Poisson noise prevails \cite{mitra2014can}, suggesting coding and compressed sensing approaches designed for effectiveness under the AGN or noiseless conditions unsuitable under Poisson noise. Existing literature strongly discourages their utilization in such situations \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. \YLnote{This issue was first identified by Mitra et al \cite{mitra2014can} but has not received significant attention.} \Xpolish{As Mitra et al. highlighted, a data-driven prior can significantly improve the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}, the cost function based on L2 error metric lacks fundamental perceptual information \cite{mitra2014can}. In this project, the primary objectives is to better identify the role of data-driven prior in computer vision tasks on a more meaningful metric, and further fix the limitations when learning that prior in provious models.}{
As emphasized by Mitra et al., leveraging a data-driven prior can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. However, the cost function based on the L2 error metric lacks essential perceptual information \cite{mitra2014can}. Our study aims to illustrating why AGN is not suitable for optimizing coding under Poisson noise by direct comparison, elucidating the nuanced impact of a data-driven prior on computer vision tasks using more meaningful metrics, and addressing limitations encountered in previous models during the learning \Xhide{process }of such priors and the optimization of coding schemes.
}

\Bingnote{{Clarity and Focus: Ensure the introduction clearly states the problem and the proposed solution. It should succinctly explain why Poisson noise is significant and how it affects imaging systems.}}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        % \centering
         \caption{Direct Measurement Strategy: Raster Scan}
        % \includesvg[width=0.637\linewidth]{\homedir/figures/Background/RasterScan2.svg}
        \includegraphics[width=1\linewidth]
        {hardware_pca_onn__figures__Background__RasterScan.pdf}
        % \caption{Non-computational Imaging scheme}
        \label{fig:RasterScan}       
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        % \centering     
        \caption{Computational Imaging (CI) Strategy: Basis Scan}
        \includegraphics[width=1\linewidth]{hardware_pca_onn__figures__Background__BasisScan.pdf}
        % \includesvg[width=0.9\linewidth]{\homedir/figures/Background/BasisScan2.svg}        
        \label{fig:BasisScan}        
    \end{subfigure}
    \caption{$\B{x}$: object, $\B{M}$: masks of coding, $\B{y}$: counted photon numbers at the sensor, $\B{M}^{-1}$: reconstruction operator, $\tilde{\B{x}}$: reconstructed object. (\subref{fig:RasterScan}) Only one pixel (white) is scanned in each measurement, and the measured data requires no reconstruction. (\subref{fig:BasisScan}) The sum of all white pixels is measured in each measurement and it requires a decoding step to reconstruct the field of view.
    }
    \label{fig:SinglePixelImaging}
\end{figure}

The \textbf{single-pixel-camera} \Xpolish{demonstrated}{shown} in Fig. \ref{fig:SinglePixelImaging} is a \Xpolish{typical}{popular} example of \Xpolish{this model}{coding}, and serves as the primary example in this project. \YLnote{It employs a rapid single-pixel detector in conjunction with a Digital Micromirror Device (DMD) to sequentially multiplex a sensing matrix by modulating various patterns on the DMD \cite{mitra2014can}.} Supposing the image representation of the field of view (FOV) $\B{x} \in \IR^{N \times 1}$ consists of $N \in \IZ^+$ pixels and is measured by $m \in \IZ^+$ \Xpolish{projections}{measurements, whose photon counts are denoted as $\B{y} \in \IR^{m \times 1}$}, 
  the single-pixel-imaging process, if ignoring noise, can be expressed as the following equation 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where \Xhide{$\B{x} \in \IR^{N \times 1}$ is the image representation of the field of view, }$\B{M} \in \IR^{m \times N}$ is a set of sensing masks linearly projecting the \Xpolish{FOV}{$\B{x}$} onto the sensor pixel\Xhide{, and $\B{y} \in \IR^{m \times 1}$ are the corresponding measured {flux} levels or photon counts }\cite{willet2009CSPoisson}. Physically, $\B{M}$ can be implemented by directing or blocking different parts of the incoming light from $\B{x}$ with masks \cite{raskar2009computational} and averaging them on sensors that digitize the detected flux levels or photon counts $\B{y}$. If the sensing matrix $\B{M}$ is full-rank, \Xpolish{this model accurately characterizes conventional single-pixel imaging scenarios}{the \Xpolish{FOV}{$\B{x}$} can be reconstructed by $\B{M}^{-1}\B{y}$}. However, even when $m < N$, \Xhide{the model remains effective through the integration of regularization techniques, specifically }{we can still recover the \Xpolish{FOV}{$\B{x}$} via} compressed sensing. \YLnote{While Hadamard matrices are considered effective for $\B{M}$, their suitability diminishes in the presence of data-dependent noise \cite{mitra2014can, harwit1979hadamard}.} In this work, we will study the performance of this camera for different choices of $\B{M}$ under different noise models. While a compressed sensing system that reconstructs an image fits this paradigm, we will focus on highly compressible problems such as character recognition. In these problems the differences between the common linear Gaussian noise model of the camera and the real Poisson noise model are most apparent.

\Bingnote{Provide a brief background on existing coding schemes and their limitations with Poisson noise. This sets the stage for the importance of your work.}

Our contributions are as listed.
\begin{itemize} 
% \item We analyze the performance of coding techniques for  using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise individually, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding \YLnote{using Hadamard and random matrices} provides no benefit over a trivial raster scanning approach under Poisson noise using an identity matrix as $\B{M}$  {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is compressible, similar benefits \Xpolish{to those seen in compressed sensing and computational imaging}{in classification rate which is more perceptually meaningful metric} can be seen if appropriate adjustments to the measurement matrices are made. 
\item We assert that coding can yield substantial performance improvements under Poisson noise \textit{only} when codes used in hardware capture are optimized specifically for downstream vision tasks, which extend beyond naive image reconstruction to include promising classification.
\item \Xpolish{We propose the methodology of selective sensing (SS) which includes coding methods selectively extracting the data-driven priors and can be directly combined with models for downstream tasks.}{We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.}
\item We provide a model to \Xpolish{create masks optimized}{optimize $\B{M}$} for Poisson noise using a neural network. \YLnote{We find optimizing measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel vision systems.} 
Addressing the limitations identified by Mitra et al. \cite{mitra2014can}, this model presents the following advantages.
    \begin{itemize}
        \item The optimization of coding relies on the gradient descent algorithm, leading to the determination of a globally optimal matrix $\B{M}$ rather than its greedy approximation.
        \item Noise is incorporated during the training process to simulate real-world conditions, deviating from the assumption of a one-dimensional affine noise model.
        \item The training process is accelerated and computationally more efficient due to the binary constraint being addressed even in real experiments. Additionally, the prior is learned from the entirety of the light fields and spectral data, rather than from patches.
        \item The contribution of a data-driven prior to performance enhancement is more accurately discerned when evaluating this model using the classification rate, a metric that holds superior interpretability in terms of visual perceptual meaning compared to the reconstruction error.
    \end{itemize}
\end{itemize}


==> hardware_pca_onn__sections__1_intro__1_intro_2024_04_01 <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi


\IEEEPARstart{O}{}ptical coding, also known as multiplexing, is a popular technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. If ignoring the noise, coding is represented as 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector, $\B{M}$ is the sensing matrix, and $\B{y}$ is the measured vector. Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$. The recovery quality of $\B{x}$, however, also depends on the conditioning of the $\B{M}$ besides the light throughput \cite{mitra2014can}. Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents Poisson noise \cite{yang2015poisson} arising intrinsically due to the discrete and random nature of photon measurements. The optimization behaviors of coding manifest notable distinctions under low-light conditions where Gaussian noise dominates and high-light conditions where Poisson noise prevails \cite{mitra2014can}, suggesting coding and compressed sensing approaches designed for effectiveness under the AGN or noiseless conditions unsuitable under Poisson noise. It has been shown that in that case without the use of priors for regularization, coding does not provide an improvement over a simple sequential scan \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}. 
Mitra et. al. \cite{mitra2014can} develop a data driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. \YLnote{An important conclusion is that if the signal exhibits sparsity and thereby  compressibility, signal optimized coding can improve recovery performance under Poisson noise and the amount of improvement is directly related to the comprehensibility of the measured data. However, recovery is typically not the ultimate goal for modern vision systems.} Furthermore, the cost function based on the L2 error metric in that project lacks essential perceptual information \cite{mitra2014can}. \YLnote{Since vision tasks, such as classification, operate in embeddings created from images their data should be inherently more compressible than their upstream imaging tasks. Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.} To show this, our study implements a simple end to end vision system that can be optimized  under different noise assumptions. We illustrate why AGN is not suitable for optimizing coding under Poisson noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when only photon noise is present.
% }

% If the signal is sparse and compressible, it is possible to have a better recovery performance under Poisson noise. However, recovery is usually not the final objective for modern vision systems. Vision tasks, such as classification, usually present greater compressibility than their upstream imaging tasks. If the signal compressibility is the answer, we should skip the intermediate imaging step and directly code for better feature extracting for next vision tasks to attain the best compressibility and therefore, better performances under Poisson noise.

Our contributions are as listed.
\begin{itemize} 
% \item We analyze the performance of coding techniques for  using toy applications in single-pixel-imaging, compare the behavior of popular approaches for both additive Gaussian and Poisson noise individually, and develop coding strategies that work under Poisson noise. 
\item Similar to the conclusion of Cossairt et al. \cite{cossairt2012does}, Mitra et al. \cite{mitra2014can}, Harwit et. al. \cite{harwit1979hadamard}, Swift et. al. \cite{swift1976hadamard}, and Raginsky et. al. \cite{willet2009CSPoisson}, we find that general prior free  coding \YLnote{using Hadamard and random matrices} provides no benefit over a trivial raster scanning approach under Poisson noise using an identity matrix\Xhide{ as $\B{M}$} {\cite{scotte2022photon_noise, wuttig2005optimal, schumann2002SNR_poisson, larson1974hadamard_poisson, streeter2009optical_poisson}}. We find, however, that in applications like compressed sensing and pattern recognition, where the collected data is highly compressible, substantial improvements in classification rate can be seen if appropriate adjustments to the measurement matrices are made. In these scenarios the compressive vision system performance approaches the performance of a non-coded camera.
\item We assert that coding can yield substantial performance improvements under Poisson noise \textit{only} when codes used in hardware capture are optimized specifically for downstream vision tasks.
\item \Xpolish{We propose the methodology of selective sensing (SS) which includes coding methods selectively extracting the data-driven priors and can be directly combined with models for downstream tasks.}{We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.}
\item We provide a model to \Xpolish{create masks optimized}{optimize $\B{M}$} for Poisson noise using neural network model. \YLnote{We find optimized measurements significantly enhances single-pixel vision performance, particularly in Poisson noise-dominated signals like visible light, approaching the efficacy of ideal multipixel vision systems.} 
Addressing the limitations identified by Mitra et al. \cite{mitra2014can}, this model presents the following advantages.
    \begin{itemize}
        \item The optimization of coding relies on the gradient descent algorithm, leading to the determination of a globally optimal $\B{M}$ rather than its greedy approximation.
        \item Noise is incorporated during the training process to simulate real-world conditions, deviating from the assumption of a one-dimensional affine noise model.
        \item The training process is accelerated and computationally more efficient due to the binary constraint being addressed even in real experiments. Additionally, the prior is learned from the entirety of the light fields and spectral data, rather than from patches.
        \item The contribution of a data-driven prior to performance enhancement is more accurately discerned when evaluating this model using the classification rate, a metric that holds superior interpretability in terms of visual perceptual meaning compared to the reconstruction error.
    \end{itemize}
\end{itemize}


==> hardware_pca_onn__sections__1_intro__1_intro_2024_04_11 <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

\AVnote{\checkednote{Lets try to make the text about machine vision system optimization. Could start with: While we have the ability to mass produce optical components of increasing complexity, creation of human interpretable imaging by closely following the optics of the human eye is still the design principle of most vision hardware. We use a single pixel camera relying on optical coding as a test bed system to optimize. This system can produce images, but allows great freedom to perform alternative measurements while being easily described mathematically.}}

% \YLnote{\IEEEPARstart{D}{}espite advances in mass-producing complex optical components, most vision systems still follow the template of human vision where the optics create a two dimensional image that is then digitized and processed. A more general imaging system that has been extensively studied is the single-pixel camera that relies on masks to perform coded measurements from which images are computed. This setup also offers flexibility for alternative measurements, with straightforward mathematical descriptions.} 


% While we have the ability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely follows the optics of the human eye to create human-interpretable imaging. However, the more generalized vision systems can also perform alternative measurement which can be easily described in mathematical ways and is more perceptually meaningful than just producing images. We use a single-pixel camera, which can be seen as a system in this kind,  relying on masks to perform coded measurements as a test bed for hardware optimization.

% can depend on direct measurement with visual perception as well. We use a single-pixel camera relying on masks to perform coded measurements from which images are computed as a test bed to optimize, as it not only can produce images but also allows great freedom to perform alternative measurements while being easily described mathematically.

\IEEEPARstart{W}{}hile we possess the capability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely mimics the optics of the human eye to create human-interpretable imaging. However, more generalized vision systems can also perform alternative coded measurements that are not only easily described mathematically but also potentially more perceptually meaningful than merely producing images. We employ a single-pixel camera as a test bed for hardware optimization, which exemplifies such a system, relying on masks to conduct optically-coded measurements. 

% Optical coding, also known as multiplexing, is a popular technology in computational imaging (CI) due to its potential to achieve enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. If ignoring the noise, coding is represented as 
%  \begin{equation}
%     \label{eqn:NoiselessMeasurement}
%     \begin{aligned}
%         \B{y} &=  \B{M x} ,
%     \end{aligned}
% \end{equation}
% where $\B{x}$ is the signal vector, $\B{M}$ is the sensing matrix, and $\B{y}$ is the measured vector. 

% Maybe: For optical coding or multiplexing an image is prjoected onto a mask and only light transmitted to the mask is collected by a single large sensor pixel. A measurement consists of a set of measurements expressed as a vector y with a set of masks. The vectiruzed masks form the rows of the measurement matrix M.

% Optical coding, or multiplexing, is a popular technology projecting an image onto a mask and collecting the light transmitting it by a large senor pixel. It potentially achieves enhanced signal-to-noise ratio (SNR) and greater light throughput than point by point measurements\cite{mitra2014can}. A measurement consists of a set of measurements expressed as a vector $\B{y}$ with a set of masks vectorized as the rows of the measurement matrix $\B{M}$. If ignoring the noise, coding is represented as 

Optical coding, or multiplexing, is a popular technology that projects an image onto a mask and collects the light transmitted through it using a large sensor pixel. It potentially achieves an enhanced signal-to-noise ratio (SNR) and greater light throughput compared to point-by-point measurements \cite{mitra2014can}. A measurement vector $\B{y}$ consists of a set of measured photon counts, with the corresponding masks vectorized as the rows of the sensing matrix $\B{M}$. Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 

Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$. The recovery quality of $\B{x}$, however, also depends on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}. Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 
%---- delete
\iffalse
{
Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN), offer a mathematically tractable framework. 
However, AGN, while suitable for modeling certain noise types introduced by measurement devices, inadequately represents \Xpolish{Poisson noise arising intrinsically due to the discrete and random nature of photon measurements}{\YLnote{\Xpolish{photon noise which arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables despite that it is indeed super-Possionian. However, we continue to use the term "Poisson noise" to maintain consistency with the terminology commonly found in the literature.}{Photon noise arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables, even though it is actually super-Poissonian. However, we continue to use the term "Poisson noise" to maintain consistency with the terminology commonly found in the literature.}}} \AVnote{\checkednote{Lets call it photon noise. Photon noise is more complex and Poisson distribution is just an approximation. Then we can explain later that the key feature to model is the fact that the variance depends on the mean.}}\cite{yang2015poisson}Past works usually distinguish between low-light regimes, where AGN introduced by imperfect sensors dominates, and bright-light regimes, where the physical photon noise dominates \cite{mitra2014can}. With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel. This reduction is significant enough that photon noise becomes the primary noise factor in the vast majority of imaging applications. }
\fi
%----
\YLnote{
Coding schemes, typically formulated under the assumption of signal-independent Additive Gaussian Noise (AGN) which arises from imperfect sensors and is introduced from the low-light regimes in many past works, offer a mathematically tractable framework. With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel. This reduction is significant enough that photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise is intrinsically signal-dependent \cite{cossairt2012does} and usually approximated by Poisson noise, even though it is actually \textbf{super-Poissonian} \cite{mandel1959fluctuations}. 
% In this work, we focus on its signal-dependent feature and propose 
% arises intrinsically due to the discrete and random nature of photon measurements and is commonly approximated by Poissonian variables. 
}
\YLnote{Unfortunately, the effects of changing the noise model are not subtle as designs that are optimal under AGN conditions often fail to approximate optimal designs under photon noise.
%
The intensity dependence of photon noise renders the camera a nonlinear system, necessitating nonlinear optimization methods. Linear optics are only truly linear in the limit of infinite photons, where quantum noise vanishes. Consequently, the linear approximation frequently used is not applicable at finite light levels.}\AVnote{\checkednote{Add here: Unfortunately, the effect of changing the noise model are not subtle. Designs optimal under AGN are usually not even approximations of optimal designs under photon noise. In fact, the intensity dependence of the noise turns the camera into a nonlinear system requiring nonlinear optimization approaches. Linear optics are only truly linear at the infinite photon limit where quantum noise disappears. The linear approximation commonly used is not applicable at any finite light level. }} 
\AVnote{\checkednote{ While this issue affects any camera optic it has been studied extensively in the context of single pixel and compressed sensing cameras that rely on coding. For example, it has been shown, that while a single pixel camera provides performance advantages under AGN, in the case of  Poisson noise that more closely resembles photon noise, coding does not ....}}  \YLnote{\Xpolish{It has been shown that in that case without the use of priors for regularization, coding does not provide an improvement over a simple sequential scan}{ While this issue impacts all camera optics, it has been extensively studied in the context of single-pixel and compressed sensing cameras that rely on coding techniques. }
For instance, although single-pixel cameras demonstrate performance advantages under AGN, coding does not offer improvements over a simple sequential scan when dealing with \Xpolish{Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}, which more closely resembles photon noise.}{photon noise, or Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.}
}
{
Mitra et al. \cite{mitra2014can} develop a data driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can}. \YLnote{An important conclusion is that if the signal exhibits sparsity and thereby  compressibility, signal optimized coding can improve recovery performance under signal-dependent noise and the amount of improvement is directly related to the comprehensibility of the measured data. However, recovery is typically not the ultimate goal for modern vision systems.}
}{
\YLnote{Since vision tasks, such as classification, operate in embeddings created from images their data should be inherently more compressible than their upstream imaging tasks. Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.} To show this, our study implements a simple end to end vision system that can be optimized  under different noise assumptions. We illustrate why AGN is not suitable for optimizing coding under \Xpolish{Poisson}{photon} noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }photon noise is present.
}

Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively. \YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}
\item \Xpolish{We provide a model to {optimize $\B{M}$} for Poisson noise using neural network model. This model is end to end vision model with classification as the performance metric}{
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

==> hardware_pca_onn__sections__1_intro__1_intro_2024_09_29 <==
\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi

\IEEEPARstart{W}{}hile we possess the capability to mass-produce optical components of increasing complexity, the design principle for most vision hardware still closely mimics the optics of the human eye to create human-interpretable imaging where the lens projects an image that is then post-processed to extract patterns.
More generalized vision systems can perform many alternative measurements that are potentially more perceptually meaningful than merely producing images. Designing such a system requires co-designing hardware and digital processing with the correct noise model.
To explore the design, we employ a single-pixel camera as a toy model for joint vision system optimization. 

The single pixel camera uses the concept of optical coding, or multiplexing, which involves projecting an image onto a mask and collecting the transmitted light with a large sensor pixel.
% We employ a single-pixel camera as a test bed for hardware optimization, which exemplifies such a system, relying on masks to conduct optically-coded measurements.
% Optical coding, or multiplexing, is a popular technology that projects an image onto a mask and collects the light transmitted through it using a large sensor pixel. 
The system can potentially achieve an enhanced signal-to-noise ratio (SNR) and greater light throughput by coding compared to point-by-point measurements \cite{mitra2014can}.
In this context, a measurement vector $\B{y}$ is formed from a set of measured photon counts, with the corresponding masks vectorized as the rows of the sensing matrix $\B{M}$.
Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 

Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$.
The recovery quality of $\B{x}$, however, also depends on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}.
Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. %The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 

% \subsection*{Transitioning from Gaussian to Photon Noise Models}
Code design is often performed under the assumption of signal-independent Additive Gaussian Noise (AGN) which arises from imperfect sensors.
With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel.
This reduction is significant enough that non-additive photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise follows a Super Poissonian distribution~\cite{mandel1959fluctuations}. For passive cameras operated with incoherent ambient light the noise can usually be approximated as Poissonian.

% \subsection*{Inapplicability of Gaussian Noise for Poisson Mask Optimization}
The transition from AGN to more realistic photon noise  fundamentally alters the designs of vision systems.
%Linear optics are only truly linear in the limit of infinite photons, where quantum noise vanishes.
%The intensity dependence of photon noise renders the camera a nonlinear system, necessitating nonlinear optimization methods. 
%Consequently, the linear approximation frequently used for AGN is not applicable at finite light levels.
%While this issue impacts all camera optics, it has been extensively studied in the context of single-pixel and compressed sensing cameras that rely on coding techniques. 
For instance, although single-pixel cameras with random masks provide performance advantages under AGN, but do not offer improvements over a simple sequential scan when dealing with  Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Furthermore, the optimal coding designs under AGN conditions fail to deliver optimal performance under photon noise. 

In response to this challenge, Mitra et al. \cite{mitra2014can} develop a data-driven prior to design optimized codes for image reconstructions that can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can} by designing measurements specifically targeting sparsity or compressibility in the data. 
%An important conclusion from their work is that if the signal exhibits sparsity and thereby compressibility, signal optimized coding can improve recovery performance under signal-dependent noise and the amount of improvement is directly related to the comprehensibility of the measured data. 

However, image recovery is typically not the ultimate goal for modern vision systems.
Since vision tasks, such as classification, operate in embeddings created from images, their data should be inherently more compressible than their upstream imaging tasks allowing for more effective measurement designs. 
%Therefore, if signal compressibility is the key, skipping the intermediate imaging step and directly focusing on coding for better feature extraction for subsequent vision tasks should yield better performance.
To show this, our study implements a simple end-to-end vision system that can be optimized  under different noise assumptions. 
We illustrate why AGN is not suitable for optimizing coding under \Xpolish{Poisson}{photon} noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }photon noise is present.


Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively for \YLnote{various downstream tasks.} \Xhide{\YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}}
\item {
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\item {
% \textbf{We train the model under the physically accurate signal-dependent photon noise, as opposed to its approximated version of Poisson noise, to enhance the robustness of our model.}
% We extend Poisson noise to an alternative approximation that places greater emphasis on signal-dependency property, using the reparameterization trick to effectively trace the gradient and train the model to be near optimal when tested under Poisson noise.
We extend Poisson noise to an alternative approximation that prioritizes the signal-dependency property, using the reparameterization trick to effectively trace the gradient and train the model to achieve near-optimal performance when evaluated under Poisson noise conditions.
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

==> hardware_pca_onn__sections__1_intro__1_intro_2024_10_29 <==
% outline
\iffalse

1. why we need co-design of hardware and software, and and use single pixel camera to demonstrate

2. what is a single pixel camera, what is coding, decoding; a bad coding can degrade the performance

3. a key factor in finding optimal coding is noise/ if no noise, no coding is needed

4. coding for poisson noise is different from coding for AGN

5. -

\fi


\iffalse
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter
file'' for ICCP 2020 submissions produced under
\LaTeX~\cite{kopka-latex} using IEEEtran.cls version 1.8b and later.
\fi


% \IEEEPARstart{W}{}hile we can mass-produce optical components of increasing complexity, most vision hardware still closely mimics the optics of the human eye to create easily interpretable images. 
% In this approach, the lens projects an image that is then post-processed to extract patterns.
% However, more generalized vision systems can perform alternative measurements that may be more perceptually meaningful than simply producing images. 
% Designing such systems requires a collaborative effort to integrate hardware and digital processing algorithms while considering the appropriate noise model.
% The significance of this approach is particularly illustrated by the single-pixel camera in this context.

% \IEEEPARstart{Optical}{}
% Optical coding is a necessary procedure in all vision systems. A suboptimal coding can 

% The single pixel camera uses the concept of optical coding, or multiplexing, which involves projecting an image onto a mask and collecting the transmitted light with a large sensor pixel.

%av added 2025-4-8
\IEEEPARstart{T}{
raditionally}, camera designs are optimized to produce human-interpretable images.
However, a camera or coded optical measurement that is optimal for reconstructing images may be sub-optimal for non-reconstruction vision tasks.
Existing optimization typically assumes additive noise, while modern optical imaging systems are mainly affected by photon noise, which is not additive. 
Previous studies have highlighted the noise model's fundamental effect on the design process outcome.

A single-pixel camera (SPC) uses the concept of optical coding, which applies an optical mask to an image, and the transmitted light is captured by a single pixel. 
Due to its simplicity and clarity, it serves as an ideal model for exploring fundamental questions related to identifying the optimal coding strategy for any vision system.
The SPC system can potentially achieve an improved signal-to-noise ratio (SNR) and higher light throughput by coding compared to point-by-point measurements \cite{mitra2014can}.
In this context, a measurement vector $\B{y}$ is formed from a set of measured photon counts, with the corresponding masks vectorized as rows of the sensing matrix $\B{M}$.
Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 
Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$.
The recovery quality of $\B{x}$
is significantly dependent on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}.
Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. 
%The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 

While a greater light throughput, or a lower noise level, can improve recovery, the improper choice of the noise model can also give rise to a suboptimal coding at specific noise levels. 
Coding design is often performed under the assumption of signal-independent additive Gaussian Noise (AGN) which arises from imperfect sensors.
With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel.
This reduction is significant enough so that nonadditive photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise follows a super-Poissonian distribution~\cite{mandel1959fluctuations}. For passive cameras operated with incoherent ambient light the noise can usually be approximated as Poissonian.

The transition from AGN to more realistic photon noise fundamentally alters the designs of vision systems.
For example, although single-pixel cameras with random masks provide performance advantages under AGN, they do not outperform a simple sequential scan when dealing with Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Moreover, this work identifies that optimal coding designs under AGN conditions do not deliver optimal performance under Poisson\Xhide{photon} noise at the same noise levels.

To address this issue, Mitra et al. \cite{mitra2014can} develop a method using data-driven priors to design optimized codes for image reconstructions. 
Their approach significantly improves the performance of coding under Poisson noise by designing measurements specifically targeting sparsity or compressibility in the data \cite{mitra2014can}. 
% It can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can} by designing measurements specifically targeting sparsity or compressibility in the data. 
However, image recovery is typically not the ultimate goal for modern vision systems.
Since vision tasks, such as classification, operate in embeddings created from images, their data should be inherently more compressible than their upstream imaging tasks, allowing for more sparsity to be exploited in measurement designs. As a result, hardware optimal for vision significantly differs from hardware optimal for imaging.
To show this, we implement a simple end-to-end vision system that can be optimized under different noise assumptions. 
We illustrate why AGN is not suitable for optimizing coding under 
% \Xpolish{Poisson}{photon}
\Xpolish{photon}{Poisson}
noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }\Xpolish{photon}{Poisson} noise is present.

Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively for \YLnote{various downstream tasks.} \Xhide{\YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}}
\item {
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\Xhide{
\item {
% are we first to use it?
We propose a hybrid optimization method for non-differentiable Poisson noise that employs AGN with signal-dependent variance and reparameterization to estimate gradients during training, while switching to Poisson noise in the testing stage for model assessment.
}
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

==> hardware_pca_onn__sections__1_intro__1_intro_2025_04_08 <==
\IEEEPARstart{O}{}ptical coding is a crucial component in all vision systems\Xpolish{. In a generalized vision system,}{, where} a measurement vector $\B{y}$ is formed from a set of measured photon counts, with the corresponding masks vectorized as rows of the sensing matrix $\B{M}$.
Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the image vector. 
Reconstruction refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$. 
The selection of a suboptimal coding design $\B{M}$ can degrade the performance of reconstruction \cite{mitra2014can}.
%add 4-9-2025
Although much research has focused on optimizing $\B{M}$ for image reconstruction, our work takes a different approach by emphasizing vision systems for specific vision tasks, an area that has been less explored. 
We show that optimizing $\B{M}$ within vision systems leads to a distinct coding design compared to traditional image reconstruction.
%add 4-9-2025
% A lot of work has been done for optimizing $\B{M}$ for image reconstruction. Differently, our work focuses on vision systems for vision tasks, and exploration in this area is not abundant. It shows that the optimization of $\B{M}$ on a vision system has different outcomes.
% so much work for imaging and M is optimized for reconstruction, but we are working on vision system, which is different
%
% The recovery quality of $\B{x}$ is significantly dependent on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}.
% Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}.
%

Traditional vision systems such as cameras use optical coding to produce human-interpretable images, with their coding designs optimized primarily for image reconstruction. 
% However, modern vision systems can be designed not just for human perception and image producing, meaning that these optimal coding designs may not deliver the best performance in more generalized non-reconstruction vision tasks.
While existing coding optimizations typically assume signal-independent additive Gaussian Noise (AGN) which arises from imperfect sensors, modern optical vision systems are mainly affected by non-additive photon noise.  
The improper choice of the noise model can also lead to suboptimal coding at specific noise levels. 
With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel.
This reduction is significant enough so that photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. 
% Photon noise follows a super-Poissonian distribution~\cite{mandel1959fluctuations}. 
For passive cameras operated with incoherent ambient light, the noise can usually be approximated as Poissonian and thus be called Poisson noise.

The transition from AGN to more realistic photon noise fundamentally alters the designs of vision systems.
For example, although single-pixel cameras with random masks provide performance advantages under AGN, they do not outperform a simple sequential scan when dealing with Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
% Moreover, this work identifies that optimal coding designs under AGN conditions do not deliver optimal performance under Poisson noise at the same noise levels.
Moreover, we show that the optimal coding designs under AGN are sub-optimal for Poisson noise at similar noise levels.

% Beyond the fact that the optimal design varies with different types of noise, we must acknowledge that image reconstruction for human perception is typically not the ultimate goal for modern vision systems.
In addition to the noise model, the optimal design also depends on the downstream machine vision task, which is not always image reconstruction.
Since vision tasks, such as classification, operate in embeddings created from images, their data should be inherently more compressible than their upstream imaging tasks, allowing for more sparsity to be exploited in measurement designs. Consequently, the hardware optimized for vision tasks differs significantly from the hardware optimized for imaging.
To show this, we implement a simple end-to-end vision system with a single-pixel camera (SPC) that can be optimized under different noise assumptions. 
% By it, we illustrate why AGN is not suitable for optimizing coding under Poisson noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the \Xpolish{optimal non-coding camera}{ideal vision system} even when Poisson noise is present.
By it, we illustrate why AGN is not suitable for optimizing coding under Poisson noise. A coding scheme optimized for a specific vision task and the correct noise model can perform nearly as well as the ideal vision system, even in the presence of Poisson noise.

Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively for \YLnote{various downstream tasks.} \Xhide{\YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}}
\item {
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.



\iffalse
\IEEEPARstart{T}{}
{raditionally}, camera designs use optical coding and decoding are optimized to produce human-interpretable images.
However, a camera or coded optical measurement that is optimal for reconstructing images may be suboptimal for non-reconstruction vision tasks.
Existing optimization typically assumes additive noise, while modern optical imaging systems are mainly affected by non-additive photon noise. 
Previous studies have highlighted the noise model's fundamental effect on the design process outcome.

A single-pixel camera (SPC) uses the concept of optical coding, which applies an optical mask to an image, and the transmitted light is captured by a single pixel. 
Due to its simplicity and clarity, it serves as an ideal model for exploring fundamental questions related to identifying the optimal coding strategy for any vision system.
The SPC system can potentially achieve an improved signal-to-noise ratio (SNR) and higher light throughput by coding compared to point-by-point measurements \cite{mitra2014can}.
In this context, a measurement vector $\B{y}$ is formed from a set of measured photon counts, with the corresponding masks vectorized as rows of the sensing matrix $\B{M}$.
Ignoring the noise, coding can be represented as
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
where $\B{x}$ is the signal vector. 
Decoding refers to the process of recovering the initial signal $\B{x}$ from $\B{y}$.
The recovery quality of $\B{x}$
is significantly dependent on the conditioning of $\B{M}$ and the light throughput of $\B{M}$~\cite{mitra2014can}.
Suboptimal $\B{M}$ have the potential to significantly degrade the performance of the vision system during the recovery process, as highlighted by Mitra et al. \cite{mitra2014can}. 
%The optimization of coding schemes regarding $\B{M}$ is intricately linked to the characteristics of noise. 

While a greater light throughput, or a lower noise level, can improve recovery, the improper choice of the noise model can also give rise to a suboptimal coding at specific noise levels. 
Coding design is often performed under the assumption of signal-independent additive Gaussian Noise (AGN) which arises from imperfect sensors.
With advances in sensor design, even the sensor noise of low-end camera sensors has been reduced to a few photons per pixel.
This reduction is significant enough so that nonadditive photon noise becomes the primary noise factor in the vast majority of imaging applications \cite{cossairt2012does}. Photon noise follows a super-Poissonian distribution~\cite{mandel1959fluctuations}. For passive cameras operated with incoherent ambient light the noise can usually be approximated as Poissonian.

The transition from AGN to more realistic photon noise fundamentally alters the designs of vision systems.
For example, although single-pixel cameras with random masks provide performance advantages under AGN, they do not outperform a simple sequential scan when dealing with Poisson noise \cite{harwit1979hadamard, swift1976hadamard, willet2009CSPoisson, scotte2022photon_noise, vanden2019various}.
Moreover, this work identifies that optimal coding designs under AGN conditions do not deliver optimal performance under Poisson\Xhide{photon} noise at the same noise levels.

To address this issue, Mitra et al. \cite{mitra2014can} develop a method using data-driven priors to design optimized codes for image reconstructions. 
Their approach significantly improves the performance of coding under Poisson noise by designing measurements specifically targeting sparsity or compressibility in the data \cite{mitra2014can}. 
% It can markedly enhance the reconstruction performance of coding schemes under Poisson noise \cite{mitra2014can} by designing measurements specifically targeting sparsity or compressibility in the data. 
However, image recovery is typically not the ultimate goal for modern vision systems.
Since vision tasks, such as classification, operate in embeddings created from images, their data should be inherently more compressible than their upstream imaging tasks, allowing for more sparsity to be exploited in measurement designs. As a result, hardware optimal for vision significantly differs from hardware optimal for imaging.
To show this, we implement a simple end-to-end vision system that can be optimized under different noise assumptions. 
We illustrate why AGN is not suitable for optimizing coding under 
% \Xpolish{Poisson}{photon}
\Xpolish{photon}{Poisson}
noise and show that a coding scheme optimized for a specific vision task and for the correct noise model can perform close to the optimal non-coding camera even when \Xhide{only }\Xpolish{photon}{Poisson} noise is present.

Our contributions are as listed.
\begin{itemize} 
\item {We introduce the methodology of Selective Sensing (SS), which encompasses coding techniques specifically designed to extract data-driven priors selectively for \YLnote{various downstream tasks.} \Xhide{\YLnote{These coding methods can be seamlessly integrated with models for downstream tasks, providing a novel approach to efficiently incorporate learned priors into various applications.\checkednote{\textbf{sales pitch?}}}}}
\item {
We provide an end-to-end vision model using classification as the performance metric, which is more perceptually meaningful than mean-squared-error (MSE), to optimize $\B{M}$.
}
\Xhide{
\item {
% are we first to use it?
We propose a hybrid optimization method for non-differentiable Poisson noise that employs AGN with signal-dependent variance and reparameterization to estimate gradients during training, while switching to Poisson noise in the testing stage for model assessment.
}
}
\end{itemize}

Our model is extendable to more general camera optics and different vision tasks in future work.

\fi

==> hardware_pca_onn__sections__1_intro__1_intro_2025_06_03 <==
% 
\YLnote{Find some place to mention Single Pixel Camera, add a contribution paragraph}


% 
% 
\YLnote{
Beyond SPAD. PMT should be mentioned as well. Or Photon Counting Techniques. Also mention it is a specific application but can be used in all camera design.
}

The development of advanced sensor technologies, particularly photon-counting sensors like Single-Photon Avalanche Diodes (SPADs), has introduced unprecedented temporal precision 
% to make them excellent candidates 
for photon-limited applications 
% such as fluorescence lifetime imaging microscopy 
\cite{ingle2019high, niehorster2016multi, antolovic2017spad, altmann2018quantum}. 
% 
% Due to the extremely low read-noise, classic computational imaging algorithms primarily designed for Additive Gaussian noise (AGN) may not present significant performance gain on SPADs \cite{cossairt2012does}. 
% %
% Conversely, Poisson noise (PN) is predominant on SPADs in most scenarios.
% 

\AVnote{
This has important implications for the design of computational imaging cameras.
Computational imaging involves modifying the camera optics by inserting masks or altering lenses to enable computational processing for improved performance. cite??? Ollie. While our findings should generalize, we will consider the single pixel camera as a simple computational imaging system. cite ???
}

\YLnote{Does FSI use single pixel camera?
Optimizing measurements for feature-specific compressive sensing \cite{neifeld2014optimizing} is using single-pixel camera, and I can say I keep using this setup in this project.
}

Because of SPADs' extremely low read-noise, signal-dependent Poisson noise (PN) dominates in most SPAD imaging scenarios including low-light-imaging, and traditional computational imaging algorithms optimized for additive Gaussian noise (AGN) may offer limited performance improvements \cite{cossairt2012does}.
%
\AVnote{
This is particularly the case when cameras are designed for machine vision and their most important performance metric is not image quality but the performance as part of a vision or pattern recognition pipeline. In this scenario, the noise model can have dramatic effects on camera design.
}
% 
To address this challenge, Cossairt et al. proposed task-specific imaging as a potential solution \cite{cossairt2012does}, which is typically equivalent to Feature-Specific Imaging.

Feature-Specific Imaging (FSI) utilizes prior knowledge about the scene and task, for example in the form of principal components obtained via principal component analysis (PCA) that are applied to the image before the light is measured and digitized. Using these coding patterns it is possible to extract features of interest before digitization, application of Poisson noise, and digital processing.
%
FSI offers benefits in reducing data burden, improving efficiency, and enhancing feature fidelity in high-AGN environments \cite{neifeld2003dual}.
% % 
% However, FSI is designed for AGN dominant cases \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}.
% %
% When PN is present, FSI is no longer the optimal 
% 
% However, since FSI is primarily designed for AGN-dominant scenarios \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}, its performance degrades in conditions where PN becomes the primary noise source, making it suboptimal in such cases.
% % 
% Therefore,
However, conventional FSI paradigms, including Neifeld et al.'s foundational work and subsequent developments, are primarily designed and optimized under AGN \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing, neifeld2008adaptive}.
% 
Its performance degrades in conditions where PN becomes the primary noise source, making it suboptimal in such cases \cite{neifeld2003dual}.
% 
% Indeed, it has been observed in early investigation in FSI that the multiplex advantages vanishes when transitioning from AGN to PN, leading to no feature fidelity enhancement compared with non-computational imaging methods \cite{neifeld2003FSI}.
Indeed, early investigations into FSI have explicitly shown that its multiplexing advantages disappear when moving from AGN to PN, resulting in no feature-fidelity improvement over conventional, non-computational imaging methods \cite{neifeld2003FSI}.
% 
Therefore, it is essential to develop new feature extraction and measurement optimization methods for FSI that are intrinsically robust to PN, moving beyond ad-hoc noise handling at the post-processing stage. 
% 
Specifically, for photon-counting sensors like SPADs, designing PN-aware algorithms for the entire FSI pipeline is becoming imperative.

In this context, we propose a Deep-Feature-Specific Imaging (DeepFSI) model to address this challenge.
% 
DeepFSI is an end-to-end model incorporating an optical-coding layer on hardware end with a deep-neural-network model on software end for specific computer vision tasks. 
% 
During the training stage, DeepFSI generates AGN and PN after the optical-coding layer, and computes the gradients under the noise to optimize it for optimal or near-optimal feature extraction via backpropagation.
% 
Unlike conventional FSI, which relies on predefined and fixed coding patterns, DeepFSI enables dynamic feature-driven coding optimization.
% 
It has been observed that DeepFSI has a better performance than conventional FSI under PN. 
% 
% Furthermore, DeepFSI has another advantage over conventional FSI which requires accurate number of features beforehand. DeepFSI has much much less performance drop when using incorrect number of features, which makes it more useful in real life.
Furthermore, unlike conventional FSI methods, which require an accurate estimate of the number of features and careful noise level estimation to avoid improper compression, DeepFSI demonstrates much greater robustness to inaccuracies in feature count. This stability not only minimizes performance degradation under mismatched conditions, but also broadens the applicability of DeepFSI beyond its specific training scenarios, enhancing its usefulness and impact in real-world applications.

% Our contributions are as listed. 
% \begin{enumerate}
%     \item We propose a noise-aware end-to-end Optical-Electronic deep networks model bridge the gap between traditional feature-specific imaging and Poisson noise.
% \end{enumerate}

The main contributions of the proposed DeepFSI model are listed below.
\begin{enumerate}
    \item Bridges the gap between traditional FSI and Poisson noise by incorporating noise generation into model training.
    \item Exceeds the limitation arising from using unsupervised methods, such as PCA, in supervised classification tasks.
    \item Enhances the robustness and performance with suboptimal assumption in application, such as varying noise level and number of masks, suggesting broader utility.
    \item Advances the computational imaging for low-read-noise sensors.
\end{enumerate}

    

==> hardware_pca_onn__sections__1_intro__1_intro_2025_07_03 <==


% 
% 
The development of advanced sensor technologies, particularly photon-counting sensors (PCS) like Single-Photon Avalanche Diodes (SPADs), has introduced unprecedented temporal precision for photon-limited applications \cite{ingle2019high, niehorster2016multi, antolovic2017spad, altmann2018quantum}. 
%
% Many attempts have been conducted using PCS for computational imaging (CI) in the pursuit of performance enhancement.
% 
PCS have been increasingly explored in computational imaging (CI) frameworks to enhance performance.
%
CI uses optical coding followed by computational decoding \cite{cossairt2012does} and the coding is traditionally designed for additive Gaussian noise (AGN). 
%
Generally, it can be expressed by 
 \begin{equation}
    \label{eqn:NoiselessMeasurement}
    \begin{aligned}
        \B{y} &=  \B{M x} ,
    \end{aligned}
\end{equation}
% $\B{y} = \B{Mx}$, 
where $\B{y}$ incorporates the measured photon numbers at sensor, $\B{M}$ is the sensing matrix of a given coding design, and $\B{x}$ is the vector representation of an image \cite{willet2009CSPoisson, cossairt2012does, harwit1979hadamard}.
%
Due to the 
% extremely low 
no read-noise on PCS, signal-dependent Poisson noise (PN) dominates in most imaging scenarios,  
% which reduces the effectiveness of such traditional CI methods on PCS \cite{cossairt2012does}.
undermining the performance gains typically achieved by such traditional CI methods \cite{cossairt2012does}.
% 
% To address this challenge, Cossairt et al. proposed task-specific imaging as a potential solution and a future direction\cite{cossairt2012does}, which is typically equivalent to Feature-Specific Imaging.
To overcome this challenge, Cossairt et al. proposed task-specific imaging, often 
exemplified by 
% equivalent to 
feature-specific imaging \cite{neifeld2003FSI}, as a promising direction for future research \cite{cossairt2012does}.

Feature-specific Imaging (FSI) utilizes prior knowledge about the scene and task, for example in the form of principal components obtained via principal component analysis (PCA) that are applied to the image before the light is measured and digitized. 
% 
Using these coding patterns, it is possible to extract features of interest before digitization, application of Poisson noise, and digital processing.
%
FSI offers benefits in reducing data burden, improving efficiency, and enhancing feature fidelity in high-AGN environments \cite{neifeld2003dual}.
% % 
% However, FSI is designed for AGN dominant cases \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}.
% %
% When PN is present, FSI is no longer the optimal 
% 
% However, since FSI is primarily designed for AGN-dominant scenarios \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}, its performance degrades in conditions where PN becomes the primary noise source, making it suboptimal in such cases.
% % 
% Therefore,
However, conventional FSI paradigms, including Neifeld et al.'s foundational work and subsequent developments, are primarily designed and optimized under AGN \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing, neifeld2008adaptive}.
% 
Its performance degrades in conditions where PN becomes the primary noise source, making it suboptimal in such cases \cite{neifeld2003dual}.
% 
% Indeed, it has been observed in early investigation in FSI that the multiplex advantages vanishes when transitioning from AGN to PN, leading to no feature fidelity enhancement compared with non-computational imaging methods \cite{neifeld2003FSI}.
Indeed, early investigations into FSI have explicitly shown that its multiplexing advantages from coding disappear when moving from AGN to PN, resulting in no feature-fidelity improvement over conventional, non-computational imaging methods \cite{neifeld2003FSI}.
% 
Therefore, it is essential to develop new feature extraction and measurement optimization methods for FSI that are intrinsically robust to PN, moving beyond ad-hoc noise handling at the post-processing stage. 
% 
Specifically, for PCS, designing PN-aware algorithms for the entire FSI pipeline is becoming imperative.

In this context, we propose a Deep Feature-specific Imaging (DeepFSI) model to address this challenge.
% 
DeepFSI is an end-to-end model incorporating an optical-coding layer on hardware end with a deep-neural-network model on software end for specific computer vision tasks. 
% 
\YLnote{
    \textbf{[R1,R2, R3]}
    % DeepFSI priortizes direct photon-efficient feature extraction instead of extraction after reconstructing full images. 
    % % 
    % In Poisson-limited regimes with fixed number of photons, allocating those photons across a greater number of measurements for reconstruction than for direct classification can lead to a drop in per-measurement SNR \cite{willet2009CSPoisson}.
    % % 
    % Without the \textbf{image then task} workflow, DeepFSI underscores the \textbf{task first} perspective, concentrating the photon budget onto a minimal set of task-relevant features, maximizing their fidelity where traditional methods would be overwhelmed by Poisson noise.
    % % 
    % It is not incompatible with reconstruction as deep networks model can be used if image recovery is the objective.
    DeepFSI priortizes direct photon-efficient feature extraction instead of feature-level analysis after full image reconstruction.
    % 
    In Poisson-limited regimes with a fixed photon budget, distributing photons across a larger number of measurements for reconstruction, instead of for direct classification, reduces the per-measurement signal-to-noise ratio (SNR) \cite{willet2009CSPoisson}.
    % 
    By removing the conventional image-then-task pipeline, DeepFSI adopts a task-first paradigm that concentrates the available photon budget only on a compact set of task-relevant features.
    % 
    This targeted allocation maximizes feature fidelity in conditions where reconstruction-based approaches are severely degraded by Poisson noise.
    % 
    Importantly, the framework remains compatible with image reconstruction objectives, as deep network models can be adapted for image recovery, e.g. U-Net, when required.
    % 
    \textbf{
    We define Feature Fidelity not as the visual similarity to the ground truth, but as the preservation of task-essential information under photon-starved conditions. In the Poisson regime, the Signal-to-Noise Ratio (SNR) of each measurement is the bottleneck. By using a classification task, we can quantitatively evaluate how well the sensing matrix captures and protects these critical features from being overwhelmed by noise. High classification accuracy is, therefore, a direct manifestation of high functional fidelity of the captured features.
    }
}
% 
During the training stage, DeepFSI simulates AGN and PN after the optical-coding layer, and computes the gradients under the noise by to optimize the coding for optimal feature extraction performance via backpropagation.
% 
Unlike conventional FSI, which relies on predefined and fixed coding patterns, 
% DeepFSI enables dynamic feature-driven coding optimization.
DeepFSI enables dynamic, data-driven coding optimized for task-specific features.
% 
% Similar to the setup in \cite{neifeld2014optimizing}, we choose a single pixel camera as the main example in simulations and experiments. 
Following the setup in \cite{neifeld2014optimizing}, we use a single-pixel camera (SPC) as the primary testbed for both simulations and experiments.
% 
The methodology developed on an SPC should be generalized to any coding-based vision systems.
%
Our results show that DeepFSI \YLnote{outperforms} conventional FSI under PN \YLnote{on extracting features for classification tasks [R3]}. 
% 
% Furthermore, DeepFSI has another advantage over conventional FSI which requires accurate number of features beforehand. DeepFSI has much much less performance drop when using incorrect number of features, which makes it more useful in real life.
Furthermore, unlike conventional FSI methods requiring an accurate estimate of the number of features and careful noise level estimation to avoid improper compression, DeepFSI demonstrates much greater robustness to inaccuracies in feature count.
% 
This stability not only minimizes performance degradation under mismatched conditions, but also broadens the applicability of DeepFSI beyond its specific training scenarios, enhancing its usefulness and impact in real-world applications.

The main contributions of the proposed DeepFSI model are listed below.
\begin{enumerate}
    \item Bridging the gap between traditional FSI and Poisson noise by incorporating noise generation into model training.
    \item Exceeding the limitation arising from using unsupervised methods, such as PCA, in supervised classification tasks.
    \item Enhancing the robustness and performance with suboptimal assumption in application, such as varying noise level and number of masks, suggesting broader utility.
    % \item Advances the computational imaging for low-read-noise sensors.
    % \YLnote{\item AGN optimal coding is not for PN}
    \item Showing that AGN-favored coding is suboptimal under PN conditions.
\end{enumerate}

\YLnote{\textbf{The novelty of DeepFSI does not reside in a specific new algorithm or sensor element, but rather in its holistic demonstration of task-prioritized photon allocation. We provide both theoretical grounding and experimental evidence that, under a fixed photon budget (Poisson regime), measuring for reconstruction is a sub-optimal use of resources. By bypassing reconstruction and learning task-specific projections directly, DeepFSI maximizes the signal-to-noise ratio (SNR) of critical features that would otherwise be buried in noise.}}

==> hardware_pca_onn__sections__2_related__2_related_2024_04_01 <==
% The works most related to our work are reviewed and listed below.
The studies most relevant to our research are summarized below.

\textbf{Coding under \Xpolish{Poisson}{photon} noise}. In \Xpolish{coded imaging}{computational imaging}, \Xhide{coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. }Hadamard matrices are considered the optimal coding scheme 
% for \Xpolish{multiplexing}{coding} 
% \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal, mitra2014can} 
in systems with only AGN \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal, mitra2014can}, although this conclusion does not hold for photon noise \cite{mitra2014can}. 
\Xpolish{However, when Poisson noise is predominant, we should not use any coding \cite{harwit1979hadamard, cossairt2012does}. When the noise is Poisson distributed, coding with sparse priors such as compressed sensing is not recommended \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}.}
{In many recent \Xpolish{projects}{works}, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance, gibson2020single, liutkus2014imaging, candes2008introduction}\YLnote{\checkednote{need more here}}, though this type of matrices are not recommended under \Xpolish{Poisson}{photon} noise\cite{willet2009CSPoisson,  willett2011poisson, vanden2019various}.
% \Xhide{ While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methods explicitly do not consider Poisson noise. Thus, the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}.}
\YLnote{Wuttig and Ratner, et al. \cite{wuttig2005optimal, ratner2007optimal} introduced \Xpolish{Poisson}{photon}-noise-aware optimization techniques for \Xpolish{multiplexing}{coding} matrices that outperform Hadamard in the presence of moderate signal-dependent noise. 
However, their analysis neglects the data priors, leading to suboptimal matrices for greater \Xpolish{Poisson}{photon} noise \cite{mitra2014can}.} Additionally, attempts at matrix optimization focusing on minimal mutual coherence \cite{mordechay2014matrixRIP} \Xpolish{lack a foundation in Poisson noise model}{do not adequately consider photon noise}, as highlighted in this study.}



% \textbf{Task Specific Imaging}


\textbf{Feature Specific Imaging}. Feature-specific imaging (FSI) is a type of imaging system \Xpolish{that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it}{where sensing matrix $\B{M}$ incorporates linear features of expected data} \cite{neifeld2003FSI, neifeld2003dual}. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}. This technique can be viewed as a variant of Compressed Sensing, in which the sensing matrix is determined based on prior information \cite{neifeld2014optimizing}. However, \Xpolish{its performance and implications under Poisson noise conditions remain relatively unexplored in the existing literature, warranting further discussion and investigation}{\YLnote{current state-of-the-art} FSI is explicitly designed for AGN rather than Poisson noise\cite{neifeld2014optimizing}}. \YLnote{FSI can be regarded as a technique that leverages data driven priors, and Mitra et al. have asserted that employing data driven priors can enhance image recovery under Poisson noise \cite{mitra2014can}. Therefore, in our work, we underscore the promising prospects of extending feature-specific concepts to a broad spectrum of vision tasks under Poisson noise.}


\textbf{End-to-end optimization}. This method \Xpolish{refers to training hardware and software networks for image processing pipelines
}{
jointly optimizes \Xpolish{camera}{optical coding} design and digital signal processing to achieve optimal overall performance
} \cite{diamond2021dirty, zhang2021deep, jacome2023middle}. \YLnote{\Xpolish{In many previous}{In previous} \Xpolish{projects}{works}, this idea was usually implemented \Xpolish{without considering Poisson noise}{without considering Poisson noise in cost functions} \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training, jacome2023middle, gibson2020single} or without optimizing masks \Xpolish{under Poisson noise during training}{with gradient incorporating Poisson distribution} \Xpolish{\cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN, gibson2020single, xu2020compressed}}{\cite{ diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN, gibson2020single, xu2020compressed}}. 
Rego et al. froze the sensing matrix as a pinhole setting without optimizing it \cite{rego2022deep}}.
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes\Xhide{ in CI}. 
\YLnote{However, Poisson noise was considered only in model testing where the most robust model was picked among a set of \Xpolish{hyper-parameter combinations}{different initialization seeds} \cite{nature2022ONN}. %supplementary note 13
Xu et al. \cite{xu2020compressed} examined the robustness of the proposed neural network model to Poisson noise\Xpolish{; however,}{, but} their training process does not explicitly incorporate the gradients affected by Poisson noise.}
As we show later, 
% however, the correct noise model is essential to obtain an optimal or near-optimal optical design.
correctly modeling the noise is crucial for achieving an optimal or near-optimal optical design.
% Tseng et al. \cite{tseng2021differentiable} proposed a general approach in end-to-end camera optimization focusing on the point-spread function and considering Poisson noise.
% In this work, we delve further in this direction, and draw the generalized methodology for all vision systems by quantitatively comparing different coding strategies, recognize the role of noise models, demonstrate the necessity of this method and demonstrate the risk if designing under a wrong hypothesis.
Our contribution in this area is developing a \Xpolish{noise-included}{noise-aware} end-to-end training approach within a neural network model to find globally optimal masks under Poisson noise for generalized vision systems beyond cameras. 
Instead of focusing on the point-spread function and camera design discussed by Tseng et al. \cite{tseng2021differentiable}, we expand the methodology to include all vision systems.
This work involves quantitative comparisons of various coding strategies, an analysis of the impact of different noise models, and an emphasis on the necessity of optimizations on hardware.
We also demonstrate the risks associated with designing under incorrect noise assumptions.
\YLnote{\Xpolish{
% these part is rewritten to avoid explaining the details
Addressing the limitations identified by Mitra et al. \cite{mitra2014can}, this model presents the following advantages.
    \begin{itemize}
        \item The optimization of coding finds a globally optimal $\B{M}$ rather than its greedy approximation.
        \item Noise is incorporated during the training process to simulate real-world conditions instead of using a one-dimensional affine noise model.
        \item The training process is accelerated and computationally more efficient as the binary constraint is addressed even in real experiments. Additionally, the prior is learned from the entirety of the light fields and spectral data, rather than from patches.
        \item The contribution of a data-driven prior to performance enhancement is more accurately discerned using the classification rate as the metric.
    \end{itemize}
}
{
Although our approach also employs data-driven priors, which is similar to that of Mitra et al., our research extends beyond \Xhide{simple }image reconstruction to address a wider spectrum of vision tasks and investigates task-specific optimization techniques on optical hardware.
% Though using data-driven priors as Mitra et.al doing, our research expands its  to encompass a broader range of vision tasks and explores optimization techniques specifically tailored for optical hardware instead of simple image reconstruction.
% Different Mitra's work which primarily uses data-driven priors for image reconstruction, our research expands its  to encompass a broader range of vision tasks and explores optimization techniques specifically tailored for optical hardware.
}
}

==> hardware_pca_onn__sections__2_related__2_related_revised_2 <==

\textbf{Coding under Poisson noise}. In coded imaging, \Xhide{coding allows the capture of a two-dimensional image with a single-pixel sensor \cite{harwit1979hadamard}. }Hadamard matrices are considered the optimal coding scheme for multiplexing \cite{harwit1979hadamard, cossairt2012does, wuttig2005optimal, mitra2014can} in systems with only AGN, though this conclusion doesn't hold for Poisson noise \cite{mitra2014can}. \Xpolish{However, when Poisson noise is predominant, we should not use any coding \cite{harwit1979hadamard, cossairt2012does}. When the noise is Poisson distributed, coding with sparse priors such as compresses sensing are not recommended \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}.}
{In many recent projects, optimization efforts focus on algorithmic enhancements for reconstruction, often maintaining the use of random coding strategies \cite{goyal2016performance, gibson2020single, liutkus2014imaging, candes2008introduction}\YLnote{\checkednote{need more here}}, though this type of matrices are not recommended under Poisson noise\cite{willet2009CSPoisson,  willett2011poisson, vanden2019various}.\Xhide{ While some approaches, such as Feature Specific Imaging (FSI), optimize sensing matrices based on learnable priors \cite{neifeld2003dual, neifeld2003FSI, neifeld2014optimizing}, these methods explicitly do not consider Poisson noise. Thus the challenge of optimizing masks under Poisson noise persists \cite{neifeld2014optimizing}.} \YLnote{Wuttig, Ratner, et al. \cite{wuttig2005optimal, ratner2007optimal} introduced Poisson noise-aware optimization techniques for multiplexing matrices, outperforming Hadamard in the presence of moderate signal-dependent noise. However, their analysis neglects data priors, leading to suboptimal matrices for greater Poisson noise \cite{mitra2014can}.} Additionally, attempts at matrix optimization focusing on minimal mutual coherence \cite{mordechay2014matrixRIP} lack a foundation in the Poisson noise model, as highlighted in this study.}



% \textbf{Task Specific Imaging}


\textbf{Feature Specific Imaging}. Feature-specific imaging (FSI) is a type of imaging system \Xpolish{that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it}{where sensing matrix $\B{M}$ incorporates linear features of expected data} \cite{neifeld2003FSI, neifeld2003dual}. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features \cite{neifeld2003FSI, neifeld2003dual, neifeld2014optimizing}. This technique can be viewed as a variant of compressed sensing, wherein the sensing matrix is determined based on prior information \cite{neifeld2014optimizing}. Nevertheless, \Xpolish{its performance and implications under Poisson noise conditions remain relatively unexplored in the existing literature, warranting further discussion and investigation}{\YLnote{current state-of-the-art} FSI is explicitly designed for AGN rather than Poisson noise\cite{neifeld2014optimizing}}. \YLnote{FSI can be regarded as a technique that leverages data driven priors, and Mitra et al. have asserted that employing data driven priors can enhance image recovery under Poisson noise \cite{mitra2014can}. Therefore, in our work, we underscore the promising prospects of extending feature-specific concepts to a broad spectrum of vision tasks under Poisson noise.}


\textbf{End-to-end optimization}. This method \Xpolish{refers to training hardware and software networks for image processing pipelines}{jointly optimizes camera design and digital signal processing to achieve optimal overall performance} \cite{diamond2021dirty, zhang2021deep, jacome2023middle}. \YLnote{In many previous projects, this idea was usually implemented \Xpolish{without considering Poisson noise}{without considering Poisson noise in cost functions} \cite{hinojosa2021learning, dun2020learned, metzler2020deep, chang2019deep, onzon2021neural, spall22hybrid_training, jacome2023middle, gibson2020single} or without optimizing masks \Xpolish{under Poisson noise during training}{with gradient incorporating Poisson distribution} \cite{tseng2021differentiable, diamond2021dirty, rego2022deep, duarte2008CS, nature2022ONN, gibson2020single, xu2020compressed}. Rego et. al froze the sensing matrix as a pinhole without optimizing it \cite{rego2022deep}}.
Wang et al. \cite{nature2022ONN} successfully implemented a neural network model for handwritten number classification on an optical device with limited photon budget, demonstrating the potential for AI-assisted optimization of coding schemes\Xhide{ in CI}. 
\YLnote{However, the Poisson noise was considered only in model testing where the most robust model was picked among a set of \Xpolish{hyper-parameter combinations}{different initialization seeds} \cite{nature2022ONN}. %supplementary note 13
Xu et al. \cite{xu2020compressed} examined the robustness of the proposed neural networks model to Poisson noise; however, the training process does not explicitly incorporate the gradients affected by Poisson noise.} Our contribution is developing a noise-\Xpolish{included}{aware} training approach within a neural network model to find the globally optimal masks under Poisson noise.

% \textcolor{blue}{Add section on feature specific imaging}



\iffalse

\YLnote{For the feature specific imaging, here are some paper to cite}

\YLnote{yizhou notes start}
\textbf{Mark A. Neifeld and Premchandra Shankar, "Feature-specific imaging," Appl. Opt. 42, 3379-3389 (2003)} Feature-specific imaging is a type of imaging system that directly measures linear features of the object irradiance distribution, instead of forming a conventional image and then extracting features from it. This approach can provide higher feature fidelity and lower detector count than conventional imaging, especially for applications that require relatively few features.  Poisson noise when the mean and variance of the photon count are equal. The paper shows that feature-specific imaging does not provide any advantage over conventional imaging in the presence of shot noise, because the shot-noise-limited SNR is inherent in the irradiance collected by the instrument and does not depend on the energy incident on any particular detector. Therefore, we can infer that feature-specific imaging would not work well with Poisson noise either, unless the mean and variance of the photon count are very different. \YLnote{However, that is where we come up with hardware PCA. We can then further reduce the text by citing Neifeld for the PCA part. }

\textbf{Abhijit Mahalanobis and Mark Neifeld, "Optimizing measurements for feature-specific compressive sensing," Appl. Opt. 53, 6108-6118 (2014)} "Although our analysis assumes that the noise is independent of the signal, this is not the case when Poisson noise is present. While a formal treatment of the effects of signal-dependent noise is beyond the scope of the paper, we compare the behavior of optimized masks to the normalized PCA in signal-dependent noise." It also has imcomplete future work "Other types of noise models will also be considered, such as signal-dependent shot noise." It seems it hasn't been studied after this paper. We could say that our contribution is designing a method to extend feature specific imaging in poisson noise model.

\YLnote{Interesting conclusions listed below}  

"FSI is a form of CS in which the measurement kernels are not random, but are based on prior knowledge of the information we are interested in sensing. Working in this FSI framework, we have developed a methodology for designing a set of masks that satisfy the photon constraint and are optimum for making measurements that minimize the reconstruction MSE in the presence of noise. "

"Of course, the primary reason for CS is to make fewer measurements than the number of pixels in the reconstructed image, and to collect the information more efficiently than a conventional image. One might intuitively expect that utilizing more features (or measurements) in the reconstruction process will yield a smaller reconstruction error. We demonstrated, however, that the photon constraint limits the number of masks that can be used at a particular SNR to reduce the reconstruction MSE. In noisy conditions, the MSE initially decreases as the number of measurements is increased, but then increases when measurements that contain more noise than signal information are included." \YLnote{It aligns with Rebecca's work.}

\textbf{W. Van den Broek, B. W. Reed, A. Béché, A. Velazco, J. Verbeeck and C. T. Koch, "Various Compressed Sensing Setups Evaluated Against Shannon Sampling Under Constraint of Constant Illumination," in IEEE Transactions on Computational Imaging, vol. 5, no. 3, pp. 502-514, Sept. 2019, doi: 10.1109/TCI.2019.2894950.}  show that for the investigated sensing matrices and in the absence of read-out noise, i.e. with only Poisson noise present, compressed sensing does not raise the amount of Fisher information in the recordings above that of a Shannon sampled signal.





\YLnote{yizhou notes end}

\ynote{andreas notes start}
Other refrerences:
M. Mordechay and Y. Y. Schechner, "Matrix optimization for poisson compressed sensing," 2014 IEEE Global Conference on Signal and Information Processing (GlobalSIP), Atlanta, GA, USA, 2014, pp. 684-688, doi: 10.1109/GlobalSIP.2014.7032205.
“Considering that the measurements are noisy, it is important to
avoid energy loss, since measurements with low energy have low
signal-to-noise ratio (SNR).”
We prove this assumption wrong in this paper ... \YLnote{ONN reconstruction}

Photon-noise: is a single-pixel camera better than point scanning? A signal-to-noise ratio analysis for Hadamard and Cosine positive modulation, Camille Scotté, Frédéric Galland1 and Hervé Rigneault
Published 7 June 2023 • © 2023 The Author(s). Published by IOP Publishing Ltd
Journal of Physics: Photonics, Volume 5, Number 3 Citation Camille Scotté et al 2023 J. Phys. Photonics 5 035003 DOI 10.1088/2515-7647/acc70b
Looking at SNR for different codes. Mostly confirms prior results. Finds that snr is improved for brightest pixels, but degraded for others. \YLnote{Only $x_i \ge k \bar{x} = \frac{k\sum_{j=1}^N x_j}{N}$ can get improved. $k$ is usually $2, 4, 16$, which means only bright pixels get reconstruction gain. E.g. cosmophotography. For normal images, that usually means the general performance degrades!}

D. Shin, J. H. Shapiro and V. K. Goyal, "Performance Analysis of Low-Flux Least-Squares Single-Pixel Imaging," in IEEE Signal Processing Letters, vol. 23, no. 12, pp. 1756-1760, Dec. 2016, doi: 10.1109/LSP.2016.2617329.
Finds bounds for noise. Probably agrees with paper above.
This is very interesting. AT very low rates the non negativity constraint can improve our estimate for multiplexing so it may become better than poisson. The paper doesn’t prove that it is better. Just says the proof for the general case is not valid and shows an experiment where an improvement is shown. Could we use the same constraint in convex optimization? What does this say about other constrained or regularized optimizations?
\ynote{andreas notes end}


\iffalse
better arrangement
coding under Poisson: mention hadamard book, ollie and becca's paper show that coding under Poiss is not ideal
mask optimization: people optimize the masks under wrong noise model, we proposed a better way for Poiss 

\fi


\YLnote{In summary, we can have a list of literature by their category
\begin{enumerate}
    \item Open more pixels doesn't help under Poisson noise (no compression): \cite{harwit1979hadamard, neifeld2003FSI, cossairt2012does, scotte2022photon_noise}
    \item Regularization doesn't help (usually comes with compression):
    \cite{willet2009CSPoisson, willett2011poisson, vanden2019various}. Their suggestion is to use fewer measurements as more measurements give rise to a greater reconstruction error upper bound. BTW, ONN are can have many measurements with low rank, which doesn't contradict to this conclusion.
    \item Feature specific imaging is designed for gaussian noise especially. It is a good way for feature preserving and reconstruction. No follow-up about the poisson. That is why we start this project.
    \item When doing a classification task, we give some higher compression by labelling. E.g, gender recognition. We only need one mask to tell the gender in the most ideal case. \textbf{It will be good to find some paper directly saying this.} As the data can be highly compressible, we can avoid dense measurements, and thus have lower error bound. Reconstruction is just a linear operation, so it doesn't matter a lot if we use Rebecca's conclusion about the upper bound, even though it is for reconstruction. 
        \begin{itemize}
        \item Think about reconstructing an image about the night sky. After using TV \textbf{re-binning}, we have two colors, black for background, and white for stars. It can be treated as a classification task as well! That is why rebecca proposed some algorithms with TV stuff: to minimize the possible amount of measurements.
    \end{itemize}
    Neifeld uses features learned from training data to do reocnstruction, that is how our idea of directly classification comes from. If we want to apply the ONN for reconstruction, it may be useful to read "RecDNN: deep neural network for image reconstruction from limited view projection data"
\end{enumerate}
}
\fi


\AVnote{\checkednote{Regularization, CS, might help but noise bounds are very unfavorable (cite becca). \\ In most of the papers, people optimize the algorithm. In only very few people try to optimize the masks. No paper where masks are optimize with poisson noise. \\ In this paper we are looking at how to optimize the measurement under poisson noise. \\ We find that optimizing the measurement can have profound improvements to the performance of single pixel vision approaching the perfonance of ideal mutipixel cameras in particular for Poisson noise dominated signals like visible light. }}




==> hardware_pca_onn__sections__4_methods__simulations__simulated_data_generation <==
\Xpolish{Two classification tasks are introduced in this section. We first test the performances of all the coding schemes on the MNIST dataset for number recognition, and then test them on the hyperspectral data.}{
In this section, we present two distinct classification tasks. 
Initially, we evaluated the effectiveness of various coding schemes using the MNIST dataset, focusing on their performance in number recognition. 
Subsequently, we extend the evaluation to hyperspectral data, examining the adaptability and efficacy of the coding schemes in this different domain. 
}


% \subsubsection{MNIST Simulated Data Preparation}

% \subsubsection{MNIST Data Pre-processing}

\Xpolish{The MNIST dataset consists of handwritten digits from 0 to 9, with a default size of 28 by 28 pixels \cite{lecun1998MNIST}. In order to align the data with the Hadamard matrices, we padded the images with black pixels at the edges to resize them to 32 by 32 pixels \cite{lecun1998MNIST}. We then transformed the range of all the pixel values from $[0,1]$ to $[0.3, 1]$. This operation enhanced the persuasiveness of the dataset for various noise models, as the added black pixels do not generate Poisson noise, whose variance is proportional to the expected photon counts. \bnote{did we ever vary the dark level (0.3)/ have results showing its effect?}}{
The MNIST dataset, which consists of handwritten digits ranging from 0 to 9, has a default size of 28 by 28 pixels \cite{lecun1998MNIST}. 
To align the data with Hadamard matrices, we add black pixels to the edges of the images and resize them to 32 by 32 pixels \cite{lecun1998MNIST}. 
Subsequently, we rescale the pixel values from the original range of $[0,1]$ to $[0.3, 1]$. This rescaling introduces non-zero Poisson noise to the black regions, which has variance proportional to the expected photon counts.
}

{
We evaluate our proposed model through simulations \Xpolish{that test}{incorporating} both AGN and Poisson noise models, using varying exposure times to generate results at different noise levels. 
We also test all {compressible} strategies, varying the total number of masks but fixing the total exposure time, and define a metric called compression ratio as the ratio of the number of masks to the number of pixels \cite{stojek2022define_compression_ratio}. 
For RS and HB, this ratio is restricted to 1.00, while the rest are evaluated over values in $\mathcal{C}_R \in \{0.01, 0.04, 0.09, 0.16, 0.25, 0.36, 0.49, 0.64, 0.81, 1.00\}$ so that $\B{M}$ of each coding scheme is not restricted to being full-rank. 
The final comparison involves only the best results among all compression ratios for each strategy. Unlike pre-defined masks used by other strategies, the initial masks for ONN can affect performance in the presence of noise. 
We therefore initialized its masks with the PCA components from the training data.
}

%% add 4-9-2025
The experiment for hyperspectral data essentially applies the same model to different tasks and follows a similar overall architecture. Detailed information and results can be found in the supplemental document.
% The work on hyperspectral data has the similar overall architecture and the details can be found in the supplemental document.

==> hardware_pca_onn__sections__4_methods__simulations__spectral_datasets <==



% \rnote{How well this model can work w/o noise}

% \subsubsection{Performance Evaluation}


\Xhide{\Xpolish{The performances of the models were evaluated through their average classification rates. To ensure a thorough assessment, the model was tested five times independently, each time with a randomly split dataset for training 70\% and validation 30\%. During each assessment, the model generated noisy photon counts, which were then used to train the classifier until the validation rate reached a plateau or declined. The best validation rate achieved during the training process was chosen as the upper bound of representative performance for each assessment. The overall performance of the model was determined by averaging the results of all five assessments.}
{The model performances were assessed based on their average classification rates, which were calculated after five independent tests. In each test, the dataset was randomly divided into 70\% for training and 30\% for validation. The model generated noisy photon counts during each assessment, and the training continued until the validation rate reached a plateau or declined. The highest validation rate obtained during the training process was considered as the representative upper bound for each assessment. The overall performance of the model was determined by averaging the results of all five assessments. This comprehensive evaluation ensured the reliability and accuracy of the model performance.}}

\Xpolish{\Xpolish{In this experiment, w}{W}e utilized the Indian Pines dataset \cite{PURR1947}, which is acquired through the Airborne Visible/Infrared Imaging Spectrometer (AVIRIS) on June 12, 1992, covering the Purdue University Agronomy farm northwest of West Lafayette and its surrounding area. Comprising $145 \times 145$ pixels and 224 spectral reflectance bands in the wavelength range of 0.4 to 2.5 $\mu m$, this dataset provides a comprehensive view of the study area. Fig. \ref{fig:pines_dataset} illustrates the classes within the Indian Pines dataset, presenting the counts associated with each class. The figure also features a representation of one channel (band 12) for all pixels, along with the ground truth of semantic labeling.}{
% text starts
We use the Indian Pines dataset \cite{PURR1947}, acquired through AVIRIS on June 12, 1992, covering the Purdue University Agronomy farm and surrounding areas. 
With $145 \times 145$ pixels and 224 spectral bands (0.4 to 2.5 $\mu m$) per pixel, this dataset offers a comprehensive view of this area. 
Fig. \ref{fig:pines_dataset} illustrates 16 classes in Indian Pines, along with their counts and semantic labeling of the ground truth. 
It features a representation of band-12 for all pixels. 
Fig. \ref{fig:AeroRIT_Histogram} shows the relative intensity of the selected classes from the spectrum data, providing a concise overview of their differences.
}

\begin{figure}[ht]
\begin{subfigure}{\linewidth}
    \caption{Indian Pines Visualization}
    \centering
    \includegraphics[width=1\linewidth]{hardware_pca_onn__figures__Results__Hyperspectra__YZ_IndianPines_dataset.pdf}
    
    \label{fig:pines_dataset}
\end{subfigure}
% \end{figure}

% \begin{figure}[h]
\begin{subfigure}{\linewidth}
\caption{Spectrum View of Indian Pines}
    \centering
    % \includegraphics[width=.8\linewidth]{hardware_pca_onn__figures__Results__Hyperspectra__IndianPines_histogram.png}
    % \caption{Spectrum for each class in the Indian Pines dataset}
    \includegraphics[width=1\linewidth]{hardware_pca_onn__figures__Results__Hyperspectra__YZ_IndianPines_histogram.pdf}
    % \caption{Average spectrum for each class in the Indian Pines dataset. Classes with data entries fewer than 400 are excluded.}
    \label{fig:AeroRIT_Histogram}
\end{subfigure}
\caption{\Xpolish{Indian Pines dataset visualization\cite{PURR1947}. The top-left figure shows the band 12 of the entire spectrum. The bottom left figure shows the classes by different colors in the legend. The legend includes the class numbers and the corresponding counts.}{(\subref{fig:pines_dataset}) Visualization of the Indian Pines dataset using Band 12 from the entire spectrum (top-left). The bottom-left figure represents classes with distinctive colors as specified in the legend, which includes class labels and their respective counts \cite{PURR1947}.} {(\subref{fig:AeroRIT_Histogram}) Average spectrum for each selected class in the Indian Pines dataset. Classes with data entries fewer than 400 are excluded. 
\Xpolish{Baselines ($10,9,\dots,0$) are shown as dashed horizontal lines under each spectrum and added to the original sprectrum for better seperate view.
}{
Baselines ($10, 9, \dots, 0$) are displayed as dashed horizontal lines beneath each spectrum and are also overlaid on the original spectrum for clearer separation.
}
}}
\end{figure}

\Xpolish{In this experiment, spectral data were zero-padded from 224 to 256 to align with the Hadamard mask and \YLnote{\Xpolish{normalized}{re-scaled}} to the range $[0,1]$. We utilized the scanner-classifier module in Fig. \ref{fig:model_config}, adapting the ONN classification layers to the new dataset sizes. Each classification ran for 2000 epochs, with a learning rate of $5 \times 10^{-3}$ and a batch size of 5000.}{
% text
\Xpolish{In the experiment, spectral data \YLnote{extracted as arrays from each pixel}, zero-padded from 224 to 256 for Hadamard mask alignment and rescaled to $[0,1]$, undergoes processing using the modified scanner-classifier module from Fig. \ref{fig:model_config}}{
% 
In the experiment, spectral data vectors, extracted as arrays from each pixel, are zero-padded from 224 to 256 in length for Hadamard mask alignment and rescaled to $[0,1]$. 
It undergoes processing using the modified scanner-classifier module illustrated in 
% Fig. \ref{fig:model_config}
main text}. 
The classifier is \Xpolish{streamlined}{simplified} into a single fully connected layer with 1478 neurons, using the default architecture provided by \texttt{scikit-learn} during the preproject testing phase which gives an 86\% classification rate without any coding or noise. 
The ONN classification layers are adjusted to accommodate input data subsets, each containing 400 entries per class. 
Classes with fewer than 400 entries are omitted to maintain an unbiased input. 
}

\Xpolish{The model performances were assessed based on their average classification rates, which were calculated after five independent tests. In each test, the dataset is randomly split into 90\% for training and 10\% for validation. The model generated noisy photon counts during each assessment, and the training continues until the validation rate reached a plateau or declined. The highest validation rate obtained during the training process is considered as the representative upper bound for each assessment. The overall model performance is determined by averaging the results from all five assessments. This comprehensive evaluation ensures the reliability and accuracy of the model performance.}{
% text
Model performance is evaluated using average classification rates from five independent tests. 
Each test involves a random 90\%-10\% training-validation split of the dataset. Training continues until the validation rate plateaued or declined, with the highest validation rate representing the upper bound for each test. 
\Xpolish{The final performance metric is the average of the five maximum validation rates, ensuring a reliable and accurate assessment of the model.}{
The final performance metric is the average of the five highest validation rates.
}
}

==> hardware_pca_onn__sections__5_results__pdfplots__MNIST_Gaussian <==
\begin{tikzpicture}
    
        \begin{myaxis}[
        title={MNIST Classification AGN},        
        xlabel={Reconstruction Error of Impulse Imaging},
        ylabel={Classification Rate},
        xmode=log,
        log basis x={10},
        ]
        
        \addplot[
            color=blue,
            mark=o,
            thick
        ] coordinates {
            (2.100e+04, 1.090e-01) (2.100e+02, 1.337e-01) (2.100e-01, 7.410e-01) (2.100e-03, 9.503e-01) (2.100e-05, 9.650e-01) (2.100e-07, 9.635e-01) (2.100e-11, 9.625e-01) (2.100e-13, 9.630e-01) 
        };
        \addlegendentry{DeepFSI}

        \addplot[
            color=red,
            mark=o,
            thick
        ] coordinates {
            (2.100e+04, 1.105e-01) (2.100e+02, 1.135e-01) (2.100e-01, 5.338e-01) (2.100e-03, 9.122e-01) (2.100e-05, 9.641e-01) (2.100e-07, 9.668e-01) (2.100e-11, 9.667e-01) (2.100e-13, 9.661e-01) 
        };
        \addlegendentry{FSI}

        \addplot[
            color=Green,
            mark=square,
            thick
        ] coordinates {
            (2.100e+04, 1.024e-01) (2.100e+02, 1.054e-01) (2.100e-01, 1.066e-01) (2.100e-03, 2.109e-01) (2.100e-05, 8.665e-01) (2.100e-07, 9.553e-01) (2.100e-11, 9.600e-01) (2.100e-13, 9.604e-01) 
        };
        \addlegendentry{Hadamard}

        \addplot[
            color=black,
            mark=square,
            thick
        ] coordinates {
            (2.100e+04, 1.100e-01) (2.100e+02, 1.075e-01) (2.100e-01, 8.014e-01) (2.100e-03, 9.519e-01) (2.100e-05, 9.631e-01) (2.100e-07, 9.634e-01) (2.100e-11, 9.630e-01) (2.100e-13, 9.628e-01) 
        };                   
        
        \addlegendentry{Impulse}  
        
        \end{myaxis}     
        
        
    \end{tikzpicture}



% \begin{figure}[h]
%     \centering
    
    
    
%     \caption{ONN vs. Hardware PCA performance across varying x-values}
% \end{figure}


==> hardware_pca_onn__sections__5_results__pdfplots__MNIST_Poisson <==
\begin{tikzpicture}
        
        \begin{myaxis}[
        title={MNIST Classification PN},        
        xlabel={Reconstruction Error of Impulse Imaging},
        ylabel={Classification Rate},
        xmode=log,
        log basis x={10},
        ]
        
        
        \addplot[
            color=blue,
            mark=o,
            thick
        ] coordinates {
            (1.200e+01, 1.303e-01) (1.200e+00, 1.974e-01) (3.790e-02, 6.033e-01) (3.790e-03, 8.878e-01) (3.790e-04, 9.589e-01) (3.770e-05, 9.667e-01) (3.790e-07, 9.637e-01) (3.790e-08, 9.641e-01) 
        };
        \addlegendentry{DeepFSI}
        
        

        \addplot[
            color=red,
            mark=o,
            thick
        ] coordinates {
            (1.200e+01, 1.199e-01) (1.200e+00, 1.530e-01) (3.790e-02, 4.796e-01) (3.790e-03, 8.165e-01) (3.790e-04, 9.320e-01) (3.770e-05, 9.604e-01) (3.790e-07, 9.658e-01) (3.790e-08, 9.651e-01) 
        };
        \addlegendentry{FSI}

        \addplot[
            color=Green,
            mark=square,
            thick
        ] coordinates {
            (1.200e+01, 1.106e-01) (1.200e+00, 1.101e-01) (3.790e-02, 1.153e-01) (3.790e-03, 2.235e-01) (3.790e-04, 6.029e-01) (3.770e-05, 8.734e-01) (3.790e-07, 9.563e-01) (3.790e-08, 9.604e-01)
        };
        \addlegendentry{Hadamard}

        \addplot[
            color=black,
            mark=square,
            thick
        ] coordinates {
            (1.200e+01, 1.673e-01) (1.200e+00, 4.638e-01) (3.790e-02, 9.006e-01) (3.790e-03, 9.489e-01) (3.790e-04, 9.610e-01) (3.770e-05, 9.627e-01) (3.790e-07, 9.621e-01) (3.790e-08, 9.631e-01)
        };
        
        \addlegendentry{Impulse}     
        
        
        \end{myaxis}     
        
        
    \end{tikzpicture}

==> hardware_pca_onn__sections__Large_figures <==

\input{hardware_pca_onn__sections__5_results__2d_classification_plots}

\input{hardware_pca_onn__sections__5_results__MNIST_Masks_visualization}


==> hardware_pca_onn__sections__biography <==



\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hardware_pca_onn__figures__biography__yizhou_lu_300ppi.jpg}}]{Yizhou Lu}
\Xhide{Biography text here.}
obtained his B.S. degree in Geochemistry from Nanjing University, China, in 2017, followed by M.S. degrees in Materials Science and Engineering and Computer Sciences from the University of Wisconsin-Madison, WI, USA, in 2019 and 2023, respectively. Currently pursuing a Ph.D. degree with the Electrical and Computer Engineering Department at the University of Wisconsin-Madison, his research interests encompass computational imaging and information theory.
\end{IEEEbiography}




\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hardware_pca_onn__figures__biography__Trevor_Seets_Headshot.png}}]{Trevor Seets}
\Xhide{Biography text here.}
received his B.S. and M.S. degree in electrical engineering from the University of Wisconsin-Madison in 2019 and 2023, respectively. He is now a Ph.D. student under Professor Andreas Velten at UW-Madison. His research interests include computational optics, statistical signal processing, and imaging.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hardware_pca_onn__figures__biography__2022-04_FGB_300dpi.png}}]{Felipe Gutierrez Barragan}
\Xhide{Biography text here.}
is a Senior Software Engineer at Ubicept. He received his B.S. (2016), M.S. (2019), and Ph.D. (2022) in Computer Sciences from the University of Wisconsin-Madison.  His Ph.D. research focused on practical modifications to SPAD-based and time-of-flight 3D cameras to reduce power consumption and data bandwidth while preserving or increasing their precision. His research interests include computational imaging, computer vision, and machine learning.
\end{IEEEbiography}

% \begin{IEEEbiographynophoto}{Ehsan Ahmadi} earned his B.S. in Computer Software Engineering from Iran University of Science and Technology, Tehran, Iran, and his M.S. in Electrical and Electronics Engineering from Southern Illinois University, Carbondale, Illinois. Currently, he is pursuing a Ph.D. in Computer Engineering at UW-Madison, focusing on Fluorescence Lifetime Imaging Microscopy (FLIM).
% \end{IEEEbiographynophoto}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hardware_pca_onn__figures__biography__ehsan_ahmadi300.png}}]{Ehsan Ahmadi}
\Xhide{Biography text here.}
earned his B.S. in Computer Software Engineering from Iran University of Science and Technology, Tehran, Iran, and his M.S. in Electrical and Electronics Engineering from Southern Illinois University, Carbondale, Illinois. Currently, he is pursuing an M.S. in Computer Engineering at UW-Madison, focusing on Fluorescence Lifetime Imaging Microscopy (FLIM).
\end{IEEEbiography}



    




\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hardware_pca_onn__figures__biography__andreas_velten300.jpeg}}]{Andreas Velten}
\Xhide{Biography text here.}
received the B.A. degree in physics from the Julius Maximilian University of Wurzburg, Wurzburg, Germany, in 2003, and the Ph.D. degree in physics from the University of New Mexico, Albuquerque, NM, in 2009. From 2010 to 2012, he was a postdoctoral research associate with the Massachusetts Institute of Technology, Cambridge, MA, USA, where he was working on high speed imaging systems that can look around
a corner using scattered light. From 2013 to 2016, he was an associate scientist with the Laboratory for Optical and Computational Instrumentation, University of Wisconsin–-Madison, Madison WI, USA, working in optics, computational imaging, and medical devices. Since 2016, he has been an associate professor with the Biostatistics and Medical Informatics, Electrical and Computer Engineering Department, University of Wisconsin–-Madison. His research focuses on performing multidisciplinary work in applied computational optics and imaging.
\end{IEEEbiography}


==> main__rebuttal__rebuttal <==
\color{red}

\textbf{Rebuttal here}

\bnote{
Insist that
\begin{enumerate}
    % \item \textbf{We are the first to study FSI on Quanta-Imaging-Sensor (QIS). We deal with Poisson noise as the QIS suffer from it.} CHANGE
    \item We want to use a simple linear projection to compress data / improve the quality of feature. Making hardware too complicated (CNN, VIT, autoencoder, KernelPCA) is not a practical way. The projection is linear, and the noise happens after projection. We are interested in how this noise model affecting the projection. We can add projection visualization.
    \item We skip the reconstruction step as we should only measure necessary features instead of reconstructing with more features and throw away some afterwards under Poisson noise.
    \item For larger resolution images, we can work with patches at certain sizes. The OViT task shows how it works with $64\times64$ images. It should also work with larger images in this way.
\end{enumerate}
}

\noindent\rule{\linewidth}{0.4pt}

\textbf{Reviewer 1}:

This work presents a novel and well-structured approach to addressing Poisson-noise challenges in feature-specific imaging (FSI) through an end-to-end deep learning framework (DeepFSI). The methodology is sound, experiments are comprehensive, and the results demonstrate clear improvements over conventional FSI, especially under Poisson-noise conditions. I think the manuscript should addressing the following question before acceptance.

1. The authors use the MLGauss model to approximate Poisson noise during training. While this enables gradient flow, how does this approximation impact performance in extremely low-light regimes, where Poisson statistics deviate significantly from Gaussian approximations? Are there any experimental validations in such regimes? Have the authors considered mixed-noise models that more accurately represent real photon-counting sensors, which often exhibit both shot noise and read noise? 
\bnote{
Add a simulation: test with Poisson vs test with MLgauss. The issue is we can barely train model under Poisson. So we train under MLGauss but test under Poisson. It means, we are not proposing the theoretical solution but a practical solution. And the results is better than other methods we compared with.\\
The photon multiplier tube doesn't apparently have read noise. It records the time when a photon came in.  
}

2. DeepFSI is compared to PCA-based FSI. Were other dimensionality reduction or feature learning methods considered? Such as autoencoders and kernel PCA. If so, why were they not included in the comparison?
\bnote{
A single layer autoencoder is similar to PCA. Multilayer autoencoder is challenging to implement on hardware. We want to use a simple linear projector to preserve enough features, which is a practical way. 
% Try Kernel PCA.
Kernel PCA (kPCA) does not produce linear components in the original pixel space, making it generally unsuitable for direct mask generation compared to standard Linear PCA.
% 
If a photon signal is $x$, it is not pratical to convert it to nonlinear $k(x)$ in real world before A/D conversion. 
}

3. The experiments focus on MNIST and CIFAR-10, which are relatively low-resolution and grayscale/RGB datasets. How would DeepFSI scale to higher-resolution data, and what modifications would be needed in the optical encoder?
\bnote{
% Single pixel cam is not ideal for large images? 
The FSI paper uses patches for larger resolution images. Like what I did with ViT.
}

4. The method is trained end-to-end for classification. Would DeepFSI be equally effective for regression or reconstruction tasks under Poisson noise, or is its advantage specific to discriminative tasks?
\bnote{
Is there a way to explain that from feature we can build images as well? Like UNet. Or the features are equivalent to images in some domain?   \\
An important reason is our work is feature-first. Reconstruction tasks generally requires more features than classifications. If reconstruct first, we need to throw away unnecessary features later. If we only measure necessary features and skip reconstruction, we don't waste photon budgets on unnecessary features and have the best SNR on necessary features. If we want a reconstruction task, we can change the architecture to a Unet and use the first linear layer as masks on hardware. \\
An important insight from this and previous works is that multiplexing/coding will not bring expected benefits under Poisson noise. Under Gaussian noise, you can measure and then classification. Under Poisson noise, the best manner is only measure necessary features.\\
PCA-based FSI is unsupervised, so it works with either classification and recovery. DeepFSI is supervised, and the task needs to be determined beforehand.
% 已有：Willett/Raginsky 等给出Poisson‑CS 的误差上界——在总强度（光子数）固定时，误差上界的强度相关项会随测量数 m 增长而变差；传统“多量测=更好”的直觉在泊松模型下不成立; recons -> bigger M
\textbf{Raginsky et al. proves that the performance degarades with the number of measurements when the total number of photons is fixed; reconstruction generally needs to measure more and throw away some features later; that is why we skip reconstruction; if the objective is to reconstruct, we can just use a Unet as decoder.}
}

\noindent\rule{\linewidth}{0.4pt}
\textbf{Reviewer 2}:

The manuscript studies the joint design of optical coding and electronic processing for a photon-limited single-pixel camera. The topic is within the scope of Optics Express, and the proposed DeepFSI framework is described with simulations and one hardware proof-of-concept.

At the same time, several key ideas in DeepFSI are close to existing work on learned optics and task-specific imaging, and the present experiments are limited in scope (MNIST and CIFAR-10 in simulation, and a small digit dataset in hardware, with only classical baselines). For publication in Optics Express, major revisions are needed to clarify the novelty with respect to previous methods, to broaden and strengthen the experimental validation, and to include stronger baselines and a more detailed analysis of the noise model.

Detailed comments on major and minor points are provided in the attached review document.

Major Weaknesses
1. The manuscript presents DeepFSI as a new framework, but many of its elements
(joint optimization of the sensing matrix and a classifier, use of a differentiable
Poisson-like noise model, and feature-specific codes for single-pixel cameras) are
closely related to existing work on learned optics and task-specific imaging. The text
does not clearly separate what is new in DeepFSI from what is already known, and
there is no explicit comparison with a representative learned-optics baseline, so the
level of conceptual novelty is not clearly established for a journal article. 


\bnote{
% The learned optics considers no Poisson noise? 
\Xhide{
\textit{\textbf{We are not studying QIS, find a paper show that FSI works with }
We are studying Quanta Imager Sensor (QIS), so it is the novelty. We first migrate the FSI to QIS. The differential is the opposite when consider Poisson noise, and add figures demonstrating it. We are not designing an algorithm to address Poisson noise. We are addressing Poisson noise since we are applying FSI onto a QIS which is primarily affected by Poisson noise. So far, I don't see any previous work about using FSI on QIS.} \\}
% 
We want to stress the novalty in supervised feature extraction before A/D conversion instead of element-level novalty.
% 
Once converted to digital signal, PN is determined, and can affect the downstream tasks. In other words, if using a non-optimal code for a task, the performance is bounded.
% 
When limited by PN, the system should distribute photons only on task-related features.
% 
\textbf{
    Also, we propose this non-reconstruction method as the optimal for photon limited cases. It is based on Raginsky's conclusion, and we maximize the overall performance by skipping the image. We treat reconstruction as the same level as classification. How isn't it novel? [No work we know is about using FSI under Poisson.]
    }
% 
% 我们不主张“元素级”新颖，而是主张**“设定级 + 整体框架级”新颖**：在Poisson 主导 + 固定光子预算（这正是现代单光子/桶检的主工况）下，把 FSI 的特征前置测量以端到端方式落到单像素/计数链路中，并给出系统的基线对比与消融，这是此前没有系统化展示过的交叉点。这也是应用研究常见的新颖性来源（方法学嫁接 + 设定变更 + 体系化验证）。 
% 同时，我们以Poisson‑CS 的误差上界为理论背景，解释为何“靠增 m”在固定光子下不占优，证明“任务优先的光子分配”在现实里更有效，这种理论‑实践闭环也属于贡献的一部分。
% willet:增加测量没用；我：增加光通量没用；好钢要用到刀刃上
}

2. The experimental validation is limited for a journal paper: simulations are restricted to
MNIST and CIFAR-10, and the hardware experiment utilizes only ten digits displayed
on a monitor with a small number of repetitions, lacking confidence intervals or
statistical analysis. To judge robustness and generality of DeepFSI, more extensive
hardware tests and at least one additional task or dataset closer to realistic
single-pixel imaging scenarios would be needed.
\bnote{
\textbf{Add eigenfaces simulations, Hyperspectrum simulations}.
\textbf{Exp are used to validate the simulated results}.
\textbf{We need to use a reconstruction mask to reconstruct the images first.}
% As a complement of FSI? FSI only tested faces. \\
Even on MNIST, it cannot be finished by 10 days. The more complicated tasks take longer. The core idea we try to explain is not a hardware performance, but the robustness of the model trained on computer when directly applied on a hardware without too much prior about brightness and optimal compression. I agree a large validation set can boost the argument. The FSI paper only proposes the system design. And we showed that DeepFSI can be less sensitive and more robust in applications. \\
I can add a self handwritten number to test.\\
The model can only be trained on computer, and the most challenging question is whether it can be deployed on a hardware.\\
We will test on more tasks in the future.\\
Our camera is time‑tagged photon‑counting system. We use it for theory validation. Considering the time and data amount, it is not practical to expand hardware tasks before due.
}

3. All baselines use classical linear codes plus a fixed MLP. There is no comparison
with stronger deep-learning baselines (for example, a CNN or ViT operating on
conventional images under the same photon budget, or an existing learned coding
method for SPCs). The effect of using the MLGauss surrogate instead of exact
Poisson noise is not analyzed. As a result, it is difficult to separate the benefits of the
proposed optical coding from the choice of network architecture and from the specific
noise model, which weakens the support for the main claims.
\bnote{
% 
% 
The FSI is used on hardware, where it aims to reduce the dimension at measurements. Using CNN or ViT are essentially better, but it needs to have an image first, which is not easy to implement on hardware. We are not proposing a better way of image processing, but a compatible way with any data-driven approches. If using a CNN/ViT, we can project the first layer on the DMD as well.
\textbf{To test a conventional image, we need to recontruct it first.}
}



\begin{itemize}
    \item Section 2, page 2, lines around 6–8. The sentence “DeepFSI … computes the
gradients under the noise by to optimize the coding for optimal feature extraction performance” has a grammar error (“by to optimize”). It would be clearer to write, for
example, “and computes the gradients under the noise to optimize the coding for
feature extraction performance.”
\bnote{Addressed}

    \item Section 3.2, page 4, lines around 19–21. The phrase “II is the supreme among all
strategies” is unusual. A more neutral wording such as “II provides the upper bound
among all strategies in this work” would be clearer and more in line with the technical
style.
\bnote{Addressed}

    \item Section 3.3, page 5, lines around 24–33. Photon noise is “approximated as PN”
and later PN is used to denote Poisson noise. It would help to state explicitly that PN
stands for Poisson noise and keep this meaning consistent, to avoid confusion
between “photon noise” and “Poisson noise.”
\bnote{Addressed}

    \item Section 4.1, page 6, lines around 19–21. The sentence “the hybrid optimization
fully replies on computer simulation” contains a typo (“replies” → “relies”). Please
correct this and consider simplifying the sentence structure.
\bnote{Addressed}

    \item Section 5.2, page 10–11, lines around 19–22. The expressions “performance
supreme” and “the truncated hadamard” are slightly awkward and mix lower/upper
case. A clearer wording could be “maximum performance” and “the truncated
Hadamard code,” keeping “Hadamard” capitalized.
\bnote{Addressed}

    \item Section 5.3, page 11, lines around 9–12. There is a duplicated word in “feasibility in
in more complicated vision tasks.” One “in” should be removed. The same sentence
is quite long; splitting it into two shorter sentences would improve readability.
\bnote{Addressed}

    \item Section 5.3–5.4, page 11–12, lines around 52–56. The phrase “supreme achieved
in training conditions” is not standard English. A possible alternative is “best
performance achieved during training.”
\bnote{Addressed}

    \item Section 5.4, page 12, lines around 21–23. The statement “DeepFSI outperforms
the other coding by a huge margin” uses informal wording. For a more neutral tone, it
could be rewritten as “DeepFSI clearly outperforms the other coding designs,”
possibly followed by the exact difference in classification rate.
\bnote{Addressed}

    \item Figures and captions, page 7–8, Fig. 2. In the caption of Fig. 2 there appears to be
an isolated number “6” before the text, which looks like a leftover label rather than
part of the caption. It would be better to remove or clarify this element.
\bnote{It is part of the figure.}
\end{itemize}

\noindent\rule{\linewidth}{0.4pt}
\textbf{Reviewer 3}:

This paper targets imaging scenarios dominated by Poisson noise in photon-counting sensors, and proposes an end-to-end optical-computational imaging framework named DeepFSI. The work demonstrates clear problem awareness and practical application value. Especially in computational imaging systems such as
single-pixel cameras, traditional feature-specific imaging methods designed under
Gaussian assumptions suffer from severe performance degradation under Poisson noise, and this problem urgently needs to be addressed. The paper presents an innovative and promising method. Experimental results show that it outperforms
traditional FSI methods in Poisson noise environments. Although there are some limitations, the overall work is solid with clear contributions and is worthy of
publication. It is recommended that the authors supplement and improve the theoretical analysis, experimental comparisons, evaluation metrics, and depth of
discussion; after revision, the manuscript can be considered for publication.

1. The abstract mentions “overcoming the limitations of unsupervised methods
(e.g., PCA) in supervised classification tasks,” but does not explicitly clarify how DeepFSI achieves this improvement or on which metrics it outperforms PCA. Quantitative comparisons are lacking.

2. The paper repeatedly refers to “traditional FSI” but does not clearly define which specific methods this term encompasses (e.g., whether it includes all
PCA-based methods, or other classical coding schemes). A systematic review of the development of FSI in the literature is missing.
\bnote{
    Traditional FSI includes those with priors (training data), and classical codes such as Hadamard don't rely on data. 
}

3. Although the MLGauss model is used to approximate Poisson noise for
convenient gradient computation, it may deviate significantly from true Poisson noise under extremely low-light conditions. The paper does not discuss the impact of this
approximation on the validity of experimental conclusions.
\bnote{
Under untra-low-light conditions, any imaging system fails.
}

4. A DMD was used to emulate fractional masks in hardware experiments, but the paper does not analyze how errors introduced by this approximation affect
classification performance, nor does it provide a systematic comparison with ideal
simulation results.
\bnote{
Will have.
}

5.The paper emphasizes that DeepFSI remains robust when the compression ratio is improperly chosen, yet experiments still rely on a predefined set of
compression ratios. No explanation is provided for automatically determining the optimal compression ratio without prior knowledge.
\bnote{
I am addressing the advantages of tolerence of DeepFSI. I assume we don't know how much compression is the best, and just picked up a compression, just like what I did in OViT. Using DeepFSI, we can prepare a set of networks with different ratios and choose from them. So the experiments is to mimicking the more realistic cases. \\
If using PCA, the best ratio is relevant to the number of photons. This information cannot be known before hand. However, DeepFSI doesn't need accurate information. 
% 
Furthermore, if we design a system with optimal compression in lab setting but want to use it in outdoors setting, it is no longer optimal. The optimal compression ratio in daylight should not work for the night, and preparing models for all different ratios is not realistic.
\\
Also, we want to test the robustness and generality. In practice, we implement a method and hope it can work with multiple cases. In this work, we chose 0.09 to design a classification-oriented vision system.
}

6.DeepFSI is described as “task-specific imaging,” but the paper does not discuss
its generalization ability across different tasks (e.g., classification, detection, reconstruction), nor does it present performance on non-classification tasks.
\bnote{similar to reviewer 1. Reconstruction/detection are generally considered as task. Reconstruction requires more features that will be threw away afterwards. So the compression relies on how many features you want to use. Think about using a ReconNet and optimizing its first layer and project it on hardware.}

7.While an end-to-end optimization approach is mentioned, DeepFSI is not
systematically compared with other recent end-to-end joint optical-computational
optimization methods (e.g., differentiable optics). 
\bnote{those methods are not designed for Poisson noise I guess.}

8.The experimental dataset is small and lacks statistical significance. Only 10 test images were used in hardware experiments, which is insufficient to support the statistical conclusion that “DeepFSI significantly outperforms other methods.” 
% \bnote{Maybe I can say this method provides a extension from FSI to QIS systems.}
\bnote{
    It is not 10 test images, but generate 50 tests from a data stream by subsampling. For each test, the data are different. We will have CI analysis.
    Some method seldom succeed on some digits. But DeepFSI is more robust.
}

9.The definition and evaluation of "feature fidelity" are not rigorous. The paper
equates classification accuracy with feature fidelity, but does not analyze feature representations (e.g., feature visualization, interpretability) or adopt other dedicated feature evaluation metrics.
\bnote{I can add feature visualization; search "can i use classification rate to show feature fidelity", "is classification rate a better metric than mse in feature fidelity measurement"
[We redefine Fidelity as functional fidelity in Intro]
}

10.The conclusion does not explicitly discuss the limitations of the proposed method. Although the constraint of the MLGauss model under extremely low-light
conditions is mentioned, other potential limitations of DeepFSI are not addressed, including training time, hardware deployment complexity, and dependency on training data size.
\bnote{I should add it this time. Some previous reviewers use my limitations to attack my work.}


\color{black}

% Rebutal here
\bnote{
\begin{itemize}
    \item $\surd$ Test Poisson vs MLGauss
    \item $\surd$ Test fractional vs 1/768
    \item $\surd\square$ CI analysis on hardware
    \item $\surd\square$ Hyperspectral data results  https://www.overleaf.com/project/64cc035d5a4a21d0a5f3f6aa 2023 Dec Old 5 results hyperspectral
    \item $\surd\square$ Feature fidelity visualization 
    \item $\surd\square$ Novelty, we have visualization on masks under PN and AGN and how they are different, previous work use differential optics, dealing with Poisson noise, but they don't claim that  we should not use masks designed under AGN assumptions for PN cases.
    % \item $\square$ A simple test of tiny latex
    \item $\surd\square$ enrich the IndianPines results
    \item $\square$ acknowledgement
    \item $\square$ Evolution of FSI
    \item $\surd\square$ R2 minors
\end{itemize}
}

% 同一物理链路与同一曝光下，方法 A 在逐类别概率上对基线的一致优势在多数曝光中达到统计显著。报告 rank‑biserial 效应量显示优势是跨类别的广谱改善，而非某一两类的偶然提升。测试目的是“从仿真到物理链路”的可用性验证：
% 10 个数字固定类别的配对设计，刻意控制了“字形多样性”，把变量集中在**现实链路（显示/光学/成像/归一化）**上。
% 这与“扩大手写体多样性”是不同维度的问题；你在验证的是物理迁移鲁棒性，而非“覆盖所有书写风格”的泛化。

% 我们的类别单位是 10 个数字（0–9），评估的是从仿真到物理链路的类级性能保持与鲁棒性；本研究不涉及“对更广泛手写风格多样性的泛化”。
% subsamples 来自同一 1 s 观测，不构成独立重复，仅用于短时稳定性展示。
% 未来工作将引入多显示器/角度/距离与多书写体以扩展分布覆盖。



